The high energy behavior of QCD: The effective action and the triple-Pomeron-vertex

We study integrations over light-cone momenta in the high energy effective action of QCD. After a review of the effective action, we arrive on a regularization mechanism from matching with QCD diagrams, which we apply to a re-derivation of the reggeized gluon and of the BFKL-equation. We study consequences of the proposed regularization on the analytic structure of 2->3 and 2->4 production amplitudes in the Multi-Regge-Kinematics. We derive a certain part of the 1-loop corrections to the production vertex and demonstrate that they yield the on-set of corrections demanded by the Steinmann-relations. The Reggeon-Particle-2-Reggeon vertex is determined and applied to the construction of various signature configurations of the production amplitudes. We extend the regularization method to states of three and four reggeized gluons and propose a supplement to the effective Lagrangian. We derive vertices for the 1-3 and 2-4 reggeized gluon transition for the elastic amplitude and verify that signature conservation is obeyed. Integral equations for the state of three and four reggeized gluons are formulated and shown to agree with a result by Bartels and Wusthoff. In a second part we investigate the high-energy behavior of QCD for different surface topologies of color graphs. After a brief review of the planar limit (bootstrap and gluon reggeization) and of the cylinder topology (BFKL) we investigate the 3-3 scattering in the triple Regge limit which belongs to the pair-of-pants topology. We re-derive the triple Pomeron vertex function and show that it belongs to a specific set of graphs in color space which we identify as the analog of the Mandelstam diagram. We then extend the study to the high-energy behavior of N=4 SYM where we find a new class of color graphs not present in QCD.

==> calc.tex <==

\chapter{Calculations}
\label{cha:calc}

Werde das Rechnen mit LaTeX probieren: Los gehts

Wende die folgende Aufspaltung an
\begin{align}
  \label{eq:4}
\Gamma^{\nu\mu}_{-} (r, p) =  \tilde{\Gamma}_{-, LR}^{\nu\mu} (r = p -q, p) - (n^-)^\mu r^\nu - p^\mu (n^-)^\nu
\end{align}
mit
\begin{align}
  \label{eq:2}
\tilde{\Gamma}_{-, LR}^{\nu\mu} = g^{\mu\nu} 2p^- - (n^-)^\mu 2q^\nu  +  (n^-)^\nu 2q^\mu + \frac{{\bm{q}}^2}{p^+} (n^-)^\mu (n^-)^\nu
\end{align}

und 
\begin{align}
 \Gamma^{\mu\nu}_{+} (p, r) =  \tilde{\Gamma}_{+, LR}^{\nu\mu} ( p ,r = p-q) - (n^+)^\mu r^\nu - p^\mu (n^-)^\nu 
\end{align}
wobei
\begin{align}
  \label{eq:1}
\tilde{\Gamma}_{+, LR}^{\mu\nu} = g^{\mu\nu} 2p^+ - (n^+)^\mu 2q^\nu  +  (n^+)^\nu 2q^\mu + \frac{{\bm{q}}^2}{p^+} (n^+)^\mu (n^+)^\nu
\end{align}
Ich berechne nun zunaechst
\begin{align}
  \label{eq:3}
\tilde{\Gamma}_{+, LR}^{\mu\nu} \tilde{\Gamma}_{-, LR}^{\mu\nu} &=
 4 \cdot 4 p^+p^- + 16 q^2 +  4\frac{{\bm{q}}^4}{p^+p^-} \notag \\
&=
 4 ( 4 p^+p^- -4  {\bm{q}}^2 +  \frac{{\bm{q}}^4}{p^+p^-})
\end{align}
und 
\begin{align}
  \label{eq:5}
&( (n^-)^\mu r^\nu + p^\mu (n^-)^\nu ) \Gamma^{\mu\nu}_{+} (p, r) 
\notag \\
&= (n^-)^\mu ( p^\mu p^+ - (n^+)^\mu p^2) + (n^-)^\nu ( r^\nu p^+ - (n^+)^\nu r^2)
\notag \\
&=p^+p^- - 2p^2  + p^+p^- - 2 (p-q^2) = 2 (p^+p^- - p^2 - (p-q)^2 )
 \end{align}
ebenso
\begin{align}
  \label{eq:6}
&( (n^+)^\mu r^\nu + p^\mu (n^+)^\nu ) \Gamma^{\mu\nu}_{-} (p, r) 
\notag \\
&= (n^+)^\mu ( p^\mu p^- - (n^-)^\mu p^2) + (n^+)^\nu ( r^\nu p^- - (n^-)^\nu r^2)
\notag \\
&=p^+p^- - 2p^2  + p^+p^- - 2 (p-q^2) = 2 (p^+p^- - p^2 - (p-q)^2 )
\end{align}
und zuletzt
\begin{align}
  \label{eq:7}
&\big[ (n^-)^\mu r^\nu + p^\mu (n^-)^\nu \big] \big[ (n^+)^\mu r^\nu + p^\mu (n^+)^\nu \big] 
\notag \\
&=
2 r^2 + 2 p^-p^+ + 2 p^2
\end{align}
Es gilt
\begin{align}
  \label{eq:8}
\Gamma_-^{\nu\mu}(r,p) \Gamma_+^{\mu\nu}(p, r) 
&= (\ref{eq:3}) - (\ref{eq:5}) - (\ref{eq:6}) - (\ref{eq:7})
\notag \\
&=
4 ( 4 p^+p^- -4  {\bm{q}}^2 +  \frac{{\bm{q}}^4}{p^+p^-}) - 2 (p^+p^- - p^2 - (p-q)^2 ) 
\notag \\
&
- 2 (p^+p^- - p^2 - (p-q)^2 ) 
- 2 \big[(p-q)^2 + 2 p^-p^+ + 2 p^2\big]
\notag \\
&= 10p^+p^- + 2p^2 + 2(p-q)^2 - 16   {\bm{q}}^2 +4  \frac{{\bm{q}}^4}{p^+p^-})
\end{align}
soweit mal der Probelauf, versuchen wir es mal ernsthaft


\section{The 1 to 3  Reggeons transition at one loop}
\label{sec:1to3regg}


\subsection{Contributions of individual diagrams}
\label{sec:diagrams}

In the following we calculate different diagrams relevant for the 1 to 3 transition. All diagrams involve a integration over the loop momentum $p$ which is not explicetly shown in the formulas and will be added whenever integration is addressed.

\subsubsection{Diagram 4RPP}



We start with the following formula derived previously. The vertex for coupling of three reggeized gluons to a gluon is given by
\begin{align}
  \label{eq:10}
g^3 \frac{f^{c_1b_1c_2} f^{c_2b_2 c_3} f^{c_3b_3 c_4}}{(p - k_1)^2 (p- k_1 - k_2)^2} \Gamma^{\mu\nu}_{3+} (p ,r) + \mbox{permutations } (1,2,3)
\end{align}
where
\begin{align}
  \label{eq:9}
\Gamma^{\mu\nu}_{3+} (p ,r)
=&
 \big[4(p^+)^2 \Gamma^{\mu\nu}_+(p, r) 
- (n^+)^\mu 3p^+(r^\nu p^+ - (n^+)^\nu r^2) 
\notag \\
& -  3p^+(p^\mu p^+ - (n^+)^\mu p^2)  (n^+)^\nu \big] 
\end{align}
where $r = p - q $ and $q = k_1 + k_2 + k_3$. First, let us determine
\begin{align}
  \label{eq:11}
\Gamma^{\mu\nu}_{3+} (p ,r) \Gamma^{\nu\mu}_{-} (r ,p) &=   \big[4(p^+)^2 \Gamma^{\mu\nu}_+(p, r)  \Gamma^{\nu\mu}_{-} (r ,p)
- 
(n^+)^\mu 3p^+(r^\nu p^+ - (n^+)^\nu r^2) \Gamma^{\nu\mu}_{-} (r ,p)
\notag \\
& - 
 3p^+(p^\mu p^+ - (n^+)^\mu p^2)  (n^+)^\nu \Gamma^{\nu\mu}_{-} (r ,p) \big] 
\notag \\
&=   \big[4(p^+)^2 \Gamma^{\mu\nu}_+(p, r)  \Gamma^{\nu\mu}_{-} (r ,p)
- 
(n^+)^\mu 3p^+  \Gamma^{\nu\mu}_{-}   r^\nu p^+ +  3p^+ r^2 \Gamma^{++}_{-} (r ,p)
\notag \\
& - 
 3p^+ p^\mu p^+  \Gamma^{\nu\mu}_{-} (r ,p)   (n^+)^\nu  + 3p^+\Gamma^{++}_{-} (r ,p)  p^2  \big] 
%\notag \\
\end{align}
note that (Block Barcelona, p13)
\begin{align}
  \Gamma^{++}_{-} (r ,p) = -4p^+(1 - \frac{{\bm{q}}^2 }{p^+p^-})
\end{align}
We thus obtain
\begin{align}
  \label{eq:12}
\Gamma^{\mu\nu}_{3+} (p ,r) \Gamma^{\nu\mu}_{-} (r ,p) 
=& %% erstes ==
 \big[4(p^+)^2\big(  10p^+p^- + 2p^2 + 2(p-q)^2 - 16   {\bm{q}}^2 +4  \frac{{\bm{q}}^4}{p^+p^-}\big)
%%%%%%%%%%%
\notag \\
&- 
(n^+)^\mu 3(p^+)^2  ( p^\mu p^- - (n^-)^\mu p^2)          % \Gamma^{\nu\mu}_{-}   r^\nu 
\notag \\
& -  12(p^+)^2 r^2   (1 - \frac{{\bm{q}}^2 }{p^+p^-})        %\Gamma^{++}_{-} (r ,p)
\notag \\
& - 
 3(p^+)^2  (n^+)^\nu     (r^\nu p^- - (n^-)^\nu r^2)    % p^\mu   \Gamma^{\nu\mu}_{-} (r ,p)   
\notag \\
&
 -12 (p^+)^2 p^2  (1 - \frac{{\bm{q}}^2 }{p^+p^-})          %\Gamma^{++}_{-} (r ,p)  
 \big] 
\notag \\ %%zweites ==
=&
 \big[4(p^+)^2 \big( 10p^+p^- + 2p^2 + 2(p-q)^2 - 16   {\bm{q}}^2 +4  \frac{{\bm{q}}^4}{p^+p^-}\big)
%%%%%%%%%%%
\notag \\
&- 
 3(p^+)^2  ( p^+ p^- - 2 p^2)          % \Gamma^{\nu\mu}_{-}   r^\nu 
\notag \\
& -  12(p^+)^2 r^2   (1 - \frac{{\bm{q}}^2 }{p^+p^-})        %\Gamma^{++}_{-} (r ,p)
\notag \\
& - 
 3(p^+)^2     (p^+ p^- - 2 r^2)    % p^\mu   \Gamma^{\nu\mu}_{-} (r ,p)   
\notag \\
&
 -12 (p^+)^2 p^2  (1 - \frac{{\bm{q}}^2 }{p^+p^-})          %\Gamma^{++}_{-} (r ,p)  
 \big] 
\end{align}
Therefore
\begin{align}
  \label{eq:12cont}
\Gamma^{\mu\nu}_{3+} (p ,r) \Gamma^{\nu\mu}_{-} (r ,p) 
=& %% erstes ==
(p^+)^2 \bigg[ 
p^+p^-(40 - 3 - 3) + (p^2 + (p-q)^2)(8 + 6 - 12 )
\notag \\
& +
 {\bm{q}}^2 (-64) + 16\frac{{\bm{q}}^4}{p^+p^-} + \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)(12)  
\bigg]
\notag \\
=& %% zweites ==
(p^+)^2 \bigg[ 
34 p^+p^- + 2 (p^2 + (p-q)^2)
\notag \\
& 
 - 64 {\bm{q}}^2  + 16\frac{{\bm{q}}^4}{p^+p^-} + 12 \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)  
\bigg]
\end{align}
which gives us 
\begin{align}
  \label{eq:13}
(4RPP) =& %% erstes ==
\big[
(-gf^{c_4ac_1})g^3 \frac{f^{c_1b_1c_2} f^{c_2b_2 c_3} f^{c_3b_3 c_4}}{(p - k_1)^2 (p- k_1 - k_2)^2} \frac{-i}{p^2} \frac{-i}{(p-q)^2}
\notag \\
& (p^+)^2 \bigg[ 
34 p^+p^- + 2 (p^2 + (p-q)^2)
%\notag \\
%& 
 - 64 {\bm{q}}^2  + 16\frac{{\bm{q}}^4}{p^+p^-} + 12 \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)  
\bigg]
% \Gamma^{\mu\nu}_{3+} (p ,r) 
\notag \\
&+ \mbox{permutations } (1,2,3)\big] 
\notag \\
=& %% zweites ==
g^4 f^{c_4ac_1}f^{c_1b_1c_2} f^{c_2b_2 c_3} f^{c_3b_3 c_4} \frac{1}{p^2(p - k_1)^2 (p- k_1 - k_2)^2 (p-q)^2 }
\notag \\
& (p^+)^2 \bigg[ 
34 p^+p^- + 2 (p^2 + (p-q)^2)
 - 64 {\bm{q}}^2  + 16\frac{{\bm{q}}^4}{p^+p^-} + 12 \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)  
\bigg]
\notag \\
&+ \mbox{permutations } (1,2,3)
\end{align}
Note added: If we use the completely summetric vertex (\ref{eq:9}) and insert it into the gluon loop, an overcounting due to the symmetry of the gluon loop occurs. One should therefore insert a factor $1/2$ in order to obtain a correct result. I will do so in the following. Furthermore I will switch to generator notation where $T^{b}_{ac} = if^{abc}$. The diagram $(4RPP)$ then reads
\begin{align}
  \label{eq:61}
 (4RRP) =& g^4  \bigg[
 \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{p^2(p - k_1)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
+ 
 \frac{ \tr(T^{a}T^{b_3}T^{b_2}T^{b_1})}{p^2(p - q+ k_1)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } \notag \\
&+ 
\frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
+ 
 \frac{ \tr(T^{a}T^{b_3}T^{b_1}T^{b_2})}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
\notag \\
&+
\frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - k_1)^2 (p- q + k_2)^2 (p-q)^2 } 
+  
\frac{ \tr(T^{a}T^{b_2}T^{b_3}T^{b_1})}{p^2(p - q+ k_1)^2 (p-  k_2)^2 (p-q)^2 }
\bigg]
\notag \\
& (p^+)^2 \bigg[ 
17 p^+p^- +  (p^2 + (p-q)^2)
 - 32 {\bm{q}}^2  + 8\frac{{\bm{q}}^4}{p^+p^-} + 6 \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)  
\bigg]
\end{align}
Note that $\tr(T^{a}T^{b}T^{c}T^{d}) = \tr(T^{d}T^{c}T^{b}T^{a})$.

\subsubsection{Diagram 4G+12}

We start with the required projection of the four gluon vertex. It can be easily obtained and is stated in Block BARCELONA, p14
\begin{align}
  \gamma^{ac_1c_2b_3, -\rho\sigma +} =&
 -ig^2 f^{ac_1e} f^{bc_2e} (2 g^{\sigma\rho} - (n^-)^\sigma (n^+)^\rho)
\notag \\
&
 -ig^2 f^{ac_2e} f^{bc_1e} (2 g^{\sigma\rho} - (n^-)^\rho (n^+)^\sigma).
\end{align}
This needs to be contracted with the vertex giving the coupling of two reggeized gluons to a gluon (eg in BARCELONA, p 3):
\begin{align}
  \label{eq:14}
(\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r) =& -ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2}\Gamma^{\mu\nu}_{2+}(p,r) + \mbox{permutations } (1,2)
\notag \\
=& %% erstes ==
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \big[
2p^+\Gamma^{\mu\nu}_+(p,r) -  (n^+)^\mu (r^\nu p^+ - (n^+)^\nu r^2) 
\notag \\
&
 -  (p^\mu p^+ - (n^+)^\mu p^2)  (n^+)^\nu
\big] + \mbox{permutations } (1,2)
\end{align}
where $r = p -k$ and $k = k_1 + k_2$. Contraction with (\ref{eq:14}) leads then to
\begin{align}
  \label{eq:16}
&-ig^2 f^{ac_1e} f^{bc_2e} (2 g^{\sigma\rho} - (n^-)^\sigma (n^+)^\rho) (\Gamma^{\rho\sigma}_{2+})^{c_1b_1b_2c_3}(p,r) 
\notag \\
&
 -ig^2 f^{ac_2e} f^{bc_1e} (2 g^{\sigma\rho} - (n^-)^\rho (n^+)^\sigma) (\Gamma^{\rho\sigma}_{2+})^{c_1b_1b_2c_3}(p,r)
%\Gamma^{\rho\sigma}_{2+}(p,r) 
\notag \\
=& %% erstes ==
-ig^2 f^{ac_1e} f^{bc_2e} \big[
2(\Gamma^{\rho\rho})^{c_1b_1b_2c_3}_{2+}(p,r)  -  (\Gamma^{+-}_{2+})^{c_1b_1b_2c_3}(p,r) 
\big] 
\notag \\
&
-ig^2 f^{ac_2e} f^{bc_1e} \big[
2(\Gamma^{\rho\rho}_{2+})^{c_1b_1b_2c_3}(p,r)  -  (\Gamma^{-+}_{2+})^{c_1b_1b_2c_3}(p,r) 
\big] 
\end{align}
We have, leaving permutation aside for a moment 
\begin{align}
  \label{eq:17}
(\Gamma^{\rho\rho}_{2+})^{c_1b_1b_2c_3}(p,r) =&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \big[
2p^+\Gamma^{\rho\rho}_+(p,r) - 2 (p^+)^2  \big]
\end{align}

We have 
\begin{align}
  \label{eq:15}
{\Gamma}_{+}^{\mu\nu} (p,r) = g^{\mu\nu} 2p^+ - (n^+)^\mu( r +  2k)^\nu  -
( p -  2k)^\mu (n^+)^\nu + \frac{{\bm{k}}^2}{p^+} (n^+)^\mu (n^+)^\nu
\end{align}
and therefore
\begin{align}
  {\Gamma}_{+}^{\rho\rho} (p,r) = D 2p^+ - 2 p^+  = 2(D-1)p^+ = 6p^+
\end{align}
where $D$ is the number of dimensions which we set in the last step to $D=4$. Note that this is not valid if we intend to work in dimensional regularization. We have
\begin{align}
  \label{eq:18}
(\Gamma^{\rho\rho}_{2+})^{c_1b_1b_2c_3}(p,r) =&-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2}  \big[4(D-1)(p^+)^2  - 2(p^+)^2\big] \notag \\
=&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} 10(p^+)^2
\end{align}
Further
\begin{align}
  \label{eq:19}
(\Gamma^{+-}_{2+})^{c_1b_1b_2c_3}(p,r) =&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \big[
2p^+\Gamma^{+-}_+(p,r) - (p^+ p^+ )  2\big]
\end{align}
and as
\begin{align}
  \Gamma^{+-}_+ (p,r) = 2p^+
\end{align}
this is
\begin{align}
  \label{eq:20}
(\Gamma^{+-}_{2+})^{c_1b_1b_2c_3}(p,r) =&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} 
2(p^+)^2 
\end{align}
and
\begin{align}
  \label{eq:21}
(\Gamma^{-+}_{2+})^{c_1b_1b_2c_3}(p,r) =&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \big[
2p^+\Gamma^{-+}_+(p,r) -  2 ( p^+)^2  
\big]
\notag \\
=&
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} 
  2 ( p^+)^2  
\end{align}
where I used $\Gamma^{-+}_+(p,r) = 2p^+$. Combining everything this leads to
\begin{align}
  \label{eq:22}
(4G+12) =& %%erstes ==
 -ig^2 f^{ac_1e} f^{b_3c_3e}(-ig^2) f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \frac{-i}{p^2}\frac{-i}{(p-k_1 -k_2)} \big[
      20(p^+)^2             %2\Gamma^{\rho\rho}_{2+}(p,r)  
  - 2(p^+)^2 % \Gamma^{+-}_{2+}(p,r) 
\big] 
\notag \\
&
-ig^2 f^{ac_1e} f^{b_3c_3e}(-ig^2) f^{c_1b_2c_2} f^{c_2 b_1 c_3} \frac{1}{(p - k_2)^2} \frac{-i}{p^2}\frac{-i}{(p-k_1 -k_2)} \big[
 20(p^+)^2  -  - 2(p^+)^2
%2\Gamma^{\rho\rho}_{2+}(p,r)  -  \Gamma^{-+}_{2+}(p,r) 
\big] 
\notag \\
=& %% zweites ==
-g^4 18(p^+)^2 \big[
 f^{eac_1}f^{c_1b_1c_2} f^{c_2b_2c_3}f^{c_3b_3e} \frac{1}{p^2 (p-k_1)^2 (p - k_1-k_2)^2}
\notag \\
& +
 f^{eac_1}f^{c_1b_2c_2} f^{c_2b_1c_3}f^{c_3b_3e} \frac{1}{p^2 (p-k_2)^2 (p - k_1-k_2)^2}
\big]
\end{align}
For the permutations in (1,2) the same applies as stated after ~(\ref{eq:13}): Including them, requires due the symmetry of the loop the inserting of a statisctical factor $1/2$. In the present case this does not lead to any modification as the permutations yield exactly the same expression as given above. Again I will write the above expression in generator notation. I find
\begin{align}
  \label{eq:62}
(4G+12) =&
-g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) }{p^2 (p-k_1)^2 (p - k_1-k_2)^2}
 +
 \frac{\tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) }{p^2 (p-k_2)^2 (p - k_1-k_2)^2}
\big]
\end{align}

\subsubsection{Diagram 4G+13 and Diagram 4G+23}

Due to the symmetry of the four-gluon vertex, 4G+13 and 4G+23 are obtained from 4G+12 by exchanging corresponding indicies
\begin{align}
  \label{eq:23}
 (4G+13) =&
-g^4 18(p^+)^2 \big[
 f^{eac_1}f^{c_1b_1c_2} f^{c_2b_3c_3}f^{c_3b_2e} \frac{1}{p^2 (p-k_1)^2 (p - k_1-k_3)^2}
\notag \\
& +
 f^{eac_1}f^{c_1b_3c_2} f^{c_2b_1c_3}f^{c_3b_2e} \frac{1}{p^2 (p-k_3)^2 (p - k_1-k_3)^2}
\big]
\end{align}
and 
\begin{align}
  \label{eq:24}
 (4G+23) =&
-g^4 18(p^+)^2 \big[
 f^{eac_1}f^{c_1b_2c_2} f^{c_2b_3c_3}f^{c_3b_1e} \frac{1}{p^2 (p-k_2)^2 (p - k_2-k_3)^2}
\notag \\
& +
 f^{eac_1}f^{c_1b_3c_2} f^{c_2b_2c_3}f^{c_3b_1e} \frac{1}{p^2 (p-k_3)^2 (p - k_2-k_3)^2}
\big]
\end{align}
In generator notation they reads as 
\begin{align}
  \label{eq:63}
(4G+13) =&
-g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) }{p^2 (p-k_1)^2 (p - k_1-k_3)^2}
 +
 \frac{\tr(T^{a}T^{b_3}T^{b_1}T^{b_2}) }{p^2 (p-k_3)^2 (p - k_1-k_3)^2}
\big]
\end{align}
and
\begin{align}
  \label{eq:64}
(4G+23) =&
-g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_2}T^{b_3}T^{b_1}) }{p^2 (p-k_2)^2 (p - k_2-k_3)^2}
 +
 \frac{\tr(T^{a}T^{b_3}T^{b_2}T^{b_1}) }{p^2 (p-k_3)^2 (p - k_2-k_3)^2}
\big]
\end{align}
\subsubsection{Diagram 3I12}

At first we require the induced vertex of the second order
\begin{align}
  \label{eq:25}
\Delta_-^{c_1c_3b_3a}(-p^-, p^- - k^-, k^-) =&ig^2 {\bm{q}}^2 \big[
\frac{f^{b_3 c_1e} f^{c_3e a}}{k^- (p^- - k^-)} + \frac{f^{b_3c_3e} f^{c_1ea}}{k^- (-p^-) }
\big] (n^-)^\mu (n^-)^\nu 2 %% verwende hier alternative Darstellung
\end{align}
where we defined $k^- \equiv k_1^- + k_2^- = -k_3^-$ and contracted already the third polarization vector $(n^-)$ with $(n^+)$.
Note that an alternative representation is given by
\begin{align}
  \label{eq:37}
\Delta_-^{c_1c_3b_3a}(-p^-, p^- - k^-, k^-) =&ig^2 {\bm{q}}^2 \big[
\frac{f^{c_3 c_1e} f^{b_3e a}}{k^- (p^- - k^-)} + \frac{f^{c_3b_3e} f^{c_1ea}}{(p^- - k^-) (-p^-) }
\big](n^-)^\mu (n^-)^\nu 2 %% verwende hier nochmal alternativere Darstellung
\end{align}
 To obtain the complete diagram we further need
\begin{align}
  \label{eq:26}
(\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r) =& -ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2}\Gamma^{\mu\nu}_{2+}(p,r) + \mbox{permutations } (1,2)
\notag \\
=& %% erstes ==
-ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} \big[
2p^+\Gamma^{\mu\nu}_+(p,r) -  (n^+)^\mu (r^\nu p^+ - (n^+)^\nu r^2) 
\notag \\
&
 -  (p^\mu p^+ - (n^+)^\mu p^2)  (n^+)^\nu
\big] + \mbox{permutations } (1,2)
\end{align}
and $r = p - k_1 - k_2 = p - k$.
Including now here the factor $1/2$ for the permutations 
\begin{align}
  \label{eq:27}
(3I12) =&
\frac{1}{2} \frac{-i}{p^2} \frac{-i}{(p-k_1 -k_2)^2} \Delta_-^{c_1c_2b_3a}(-p^-, p^- - k^-, k^-) (\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r)
\end{align}
i.e. we need to evaluate
\begin{align}
  \label{eq:28}
&\Delta_-^{c_1c_2b_3a}(-p^-, p^- - k^-, k^-) (\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r) 
=
\notag \\
&ig^2 2{\bm{q}}^2 \big[
\frac{f^{c_1c_2e} f^{b_3e a}}{(-p^-)(k^-)} + \frac{f^{c_1b_3e} f^{c_3ea}}{(-p^-) (p^- - k^-)} 
\big](\Gamma^{--}_{2+})^{c_1b_1b_2c_3}(p,r) 
\end{align}
and leaving permutations aside for a while
\begin{align}
  \label{eq:29}
(\Gamma^{--}_{2+})(p,r) =& \big[
2p^+\Gamma^{--}_+(p,r) -  2[(p^- - k^-) p^+ - 2 r^2]
%\notag \\
%&
 -  (p^- p^+ - 2 p^2)  2
\big]
\end{align}
we have (\ref{eq:15})
\begin{align}
  \label{eq:30}
{\Gamma}_{+}^{--} (p,r) =&  - 2( p^- -k^- + 2 k^-)  -
( p^- -  2k^-) 2 + 4\frac{{\bm{k}}^2}{p^+} 
\notag \\
=&
- 4 p^-  +  2k^-   + 4\frac{{\bm{k}}^2}{p^+} 
\end{align}
and therefore
\begin{align}
  \label{eq:31}
(\Gamma^{--}_{2+})(p,r) =& \big[
2p^+(- 4 p^-  +  2k^-   + 4\frac{{\bm{k}}^2}{p^+}  )   -  4 p^- p^+ + 2p^+k^- + 4 (p-k)^2  + 4 p^2  
\big]
\notag \\
=&p^+ \big[-12 p^- +6k^- +    8\frac{{\bm{k}}^2}{p^+}  + 4 \frac{p^2  + (p-k)^2}{p^+} \big]
\notag \\
=&2p^+ \big[-6 p^- +3 k^- +    4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big].
\end{align}
Then
\begin{align}
  \label{eq:32}
&\Delta_-^{c_1c_2b_3a}(-p^-, p^- - k^-, k^-) (\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r) = %% erstes ==
 \notag \\
&
 -ig^2 f^{c_1b_1c_2} f^{c_2 b_2 c_3} \frac{1}{(p - k_1)^2} 
%%Delta 
ig^2 {\bm{q}}^2 \big[
\frac{f^{b_3 c_1e} f^{c_3e a}}{k^- (p^- - k^-)} + \frac{f^{b_3c_3e} f^{c_1ea}}{k^- (-p^-) } 
\big]2 \cdot
\notag \\
&
2p^+ \big[-6 p^- +3k^- +    4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big]
\notag \\
=& %% zweites ==
g^4  {\bm{q}}^2\frac{1}{(p - k_1)^2}
4p^+ \big[-6 p^- +3k^- +    4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big]
\notag \\
& \big[
-f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \frac{1}{(p^- - k^-)k^-} - f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \frac{1}{k^-(-p^-)}
\big]
\end{align}
%The full diagram (including permutations is then given by)
%\begin{align}
%  \label{eq:34}
%(3I12) =& \frac{-1}{2} \frac{-i}{p^2} \frac{-i}{(p-k_1 -k_2)^2} g^4  {\bm{q}}^2
%\frac{1}{(p - k_1)^2}
%8p^+ \big[-3 p^- +k^- +   + 2\frac{{\bm{k}}^2}{p^+}  +  \frac{p^2  + (p-k)^2}{p^+} \big]
%\notag \\
%& \big[
% f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \big(
%\frac{1}{(p^- - k^-)k^-}  +  \frac{1}{k^-(-p^-)}  \big)
%+ \mbox{permutations (1,2)}
%\big]
%\notag \\
%=&
%4p^+ \frac{1}{p^2} \frac{1}{}
%\end{align}

Note
\begin{align}
  \label{eq:33}
(-6 p^- +3k^-) \frac{1}{(p^- - k^-)k^-} 
&= 
-3( 2p^- -k^-) \frac{1}{(p^- - k^-)(k^-)}
\notag \\
&= 
-3[2 (p^- - k^-) +k^-] \frac{1}{(p^- - k^-)(k^-)}
\notag \\
&=
-3\big[
\frac{2}{k^-} + \frac{1}{p^- - k^-}
\big] = 
\big[
\frac{6}{-k^-} + \frac{3}{-p^- + k^-}
\big]
\end{align}

and
\begin{align}
  \label{eq:35}
(-6p^- + 3k^-)\frac{1}{k^-(-p^-)} = \frac{6}{k^-} - \frac{3}{p^-}
\end{align}
This yields
\begin{align}
  \label{eq:36}
&\Delta_-^{c_1c_2b_3a}(-p^-, p^- - k^-, k^-) (\Gamma^{\mu\nu}_{2+})^{c_1b_1b_2c_3}(p,r) = %% erstes ==
g^4  {\bm{q}}^2\frac{4p^+}{(p - k_1)^2}
\notag \\
&\big[
-f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \big(
\frac{6}{-k^-} + \frac{3}{-p^- + k^-}
\big) 
- f^{eac_3}f^{c_3b_1c_2}f^{c_{2}b_2 c_1}f^{c_1b_3e} \big(
 \frac{6}{k^-} - \frac{3}{p^-}
\big)
\notag \\
&
-\big(4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big) \cdot
\notag \\ 
& \big(
f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \frac{1}{(p^- - k^-)k^-} + f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \frac{1}{k^-(-p^-)}
\big)
\big]
\end{align}
The complete diagram is then given by
\begin{align}
  \label{eq:38}
(3I12) =&
\frac{1}{2} \frac{-i}{p^2} \frac{-i}{(p-k_1 -k_2)^2}  g^4  {\bm{q}}^2\frac{4p^+}{(p - k_1)^2}
\notag \\
&\big[
-f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \big(
\frac{6}{-k^-} - \frac{3}{p^- - k^-}
\big) 
- f^{eac_3}f^{c_3b_1c_2}f^{c_{2}b_2 c_1}f^{c_1b_3e} \big(
 \frac{6}{k^-} - \frac{3}{p^-}
\big)
\notag \\
&
-\big(4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big) \cdot
\notag \\ 
& \big(
f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \frac{1}{(p^- -k^-)k^-} + f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \frac{1}{k^-(-p^-)}
\big)
\big]
\notag \\
&+ \mbox{permutations (1,2)} \notag \\
=& %% zweites ==
- g^4  {\bm{q}}^2  \frac{1}{p^2} \frac{1}{(p-k)^2}  \frac{2p^+}{(p - k_1)^2}
\notag \\
&\big[
-f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \big(
\frac{6}{-k^-} - \frac{3}{p^- - k^-}
\big) 
- f^{eac_3}f^{c_3b_1c_2}f^{c_{2}b_2 c_1}f^{c_1b_3e} \big(
 \frac{6}{k^-} - \frac{3}{p^-}
\big)
\notag \\
&
-
 \big(
f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \frac{1}{(p^- - k^-)k^-} + f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \frac{1}{k^-(-p^-)}
\big) 
\notag \\
&\qquad \qquad \qquad
\cdot \big(4\frac{{\bm{k}}^2}{p^+}  +  2\frac{p^2  + (p-k)^2}{p^+} \big)  + \mbox{permutations (1,2)}
\big]
\end{align}
We attach now labels to $k$ such that $k \equiv k_{12} = k_1 + k_2$. The diagram then reads
\begin{align}
  \label{eq:39}
(3I12) =&
 g^4  {\bm{q}}^2  \frac{1}{p^2} \frac{1}{(p-k_{12})^2}  \frac{2p^+}{(p - k_1)^2}
\notag \\
&\big[
f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \big(
\frac{6}{-k_{12}^-} - \frac{3}{p^- - k_{12}^-}
\big) 
+ f^{eac_3}f^{c_3b_1c_2}f^{c_{2}b_2 c_1}f^{c_1b_3e} \big(
 \frac{6}{k_{12}^-} - \frac{3}{p^-}
\big)
\notag \\
&
+
 \big(
f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_1 c_1}f^{c_1b_3e} \frac{1}{(p^- - k_{12}^-)k_{12}^-} + f^{eac_1}f^{c_1b_1c_2}f^{c_2b_2c_3}f^{c_3b_3 e} \frac{1}{k_{12}^-(-p^-)}
\big) 
\notag \\
&\qquad \qquad \qquad
\cdot \big(4\frac{{\bm{k}}_{12}^2}{p^+}  +  2\frac{p^2  + (p-k_{12})^2}{p^+} \big)  + \mbox{permutations (1,2)}
\big]
\end{align}
In the generator notation the expression reads as 
\begin{align}
  \label{eq:76}
(3I12) =&
   \frac{ g^4  {\bm{q}}^2}{p^2(p-k_1 - k_2)^2} &&\bigg\{
\notag \\
&\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
&&\bigg[ \frac{2p^+}{(p - k_1)^2}
\bigg(
\frac{6}{k_1^- + k_2^-} + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p - k_2)^2}
 \bigg(
 \frac{6}{-k_1^- - k_2^-} - \frac{3}{p^- - k_1^- - k_2^-}\bigg)
\notag \\
&&&
+
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(-p^- )(k_1^- + k_2^-)}  
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_{1} - k_2)^2}{p^+} \bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_2)^2}
\frac{1}{(k_1^- + k_2^-)(p^--k_1^- - k_2^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad \bigg(4\frac{({\bm{k}}_{1}+ {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_1 - k_2)^2}{p^+} \bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
&&\bigg[ \frac{2p^+}{(p - k_1)^2}
\bigg( 
\frac{6}{-k_1^- - k_2^-} - \frac{3}{p^- - k_1^- - k_2^-}
\bigg) 
+
 \frac{2p^+}{(p - k_2)^2}
\bigg(
 \frac{6}{k_1^- + k_2^-} + \frac{3}{-p^-}
\bigg)
\notag \\
&&& +
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(p^- - k_1^- - k_2^-)(k_{1}^- + k_2^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad 
 \bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_1 - k_2)^2}{p^+}  
\bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_2)^2}
\frac{1}{(k_{1}^- + k_2^-)(-p^-)} 
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_{1} - k_2)^2}{p^+} \bigg)
\bigg]
\end{align}

\subsubsection{Diagrams 3I13 and 3I23}

The corresponding expresssion are due to the (bosonic) symmetry of the induced vertices obtained from (\ref{eq:39})  by exchanging corresponding labels:
\begin{align}
  \label{eq:40}
(3I13) =&
 g^4  {\bm{q}}^2  \frac{1}{p^2} \frac{1}{(p-k_{13})^2}  \frac{2p^+}{(p - k_1)^2}
\notag \\
&\big[
f^{eac_3}f^{c_3b_3c_2}f^{c_{2}b_1 c_1}f^{c_1b_2e} \big(
\frac{6}{-k_{13}^-} - \frac{3}{p^- - k_{13}^-}
\big) 
+ f^{eac_3}f^{c_3b_1c_2}f^{c_{2}b_3 c_1}f^{c_1b_2e} \big(
 \frac{6}{k_{13}^-} - \frac{3}{p^-}
\big)
\notag \\
&
+
 \big(
f^{eac_3}f^{c_3b_3c_2}f^{c_{2}b_1 c_1}f^{c_1b_2e} \frac{1}{(p^- - k_{13}^-)k_{12}^-} + f^{eac_1}f^{c_1b_1c_2}f^{c_2b_3c_3}f^{c_3b_2 e} \frac{1}{k_{13}^-(-p^-)}
\big) 
\notag \\
&\qquad \qquad \qquad
\cdot \big(4\frac{{\bm{k}}_{13}^2}{p^+}  +  2\frac{p^2  + (p-k_{13})^2}{p^+} \big)  + \mbox{permutations (1,3)}
\big]
\end{align}
and
\begin{align}
  \label{eq:41}
(3I23) =&
 g^4  {\bm{q}}^2  \frac{1}{p^2} \frac{1}{(p-k_{23})^2}  \frac{2p^+}{(p - k_2)^2}
\notag \\
&\big[
f^{eac_3}f^{c_3b_3c_2}f^{c_{2}b_2 c_1}f^{c_1b_1e} \big(
\frac{6}{-k_{23}^-} - \frac{3}{p^- - k_{23}^-}
\big) 
+ f^{eac_3}f^{c_3b_2c_2}f^{c_{2}b_3 c_1}f^{c_1b_1e} \big(
 \frac{6}{k_{23}^-} - \frac{3}{p^-}
\big)
\notag \\
&
+
 \big(
f^{eac_3}f^{c_3b_3c_2}f^{c_{2}b_2 c_1}f^{c_1b_1e} \frac{1}{(p^- - k_{23}^-)k_{12}^-} + f^{eac_1}f^{c_1b_2c_2}f^{c_2b_3c_3}f^{c_3b_1 e} \frac{1}{k_{23}^-(-p^-)}
\big) 
\notag \\
&\qquad \qquad \qquad
\cdot \big(4\frac{{\bm{k}}_{23}^2}{p^+}  +  2\frac{p^2  + (p-k_{23})^2}{p^+} \big)  + \mbox{permutations (2,3)}
\big]
\end{align}
Also the generator version is easily obtained. It is given by
\begin{align}
  \label{eq:77}
(3I13) =&
   \frac{ g^4  {\bm{q}}^2}{p^2(p-k_1 - k_3)^2} &&\bigg\{
\notag \\
&\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
&&\bigg[ \frac{2p^+}{(p - k_1)^2}
\bigg(
\frac{6}{k_1^- + k_3^-} + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p - k_3)^2}
 \bigg(
 \frac{6}{-k_1^- - k_3^-} - \frac{3}{p^- - k_1^- - k_3^-}\bigg)
\notag \\
&&&
+
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(-p^- )(k_1^- + k_3^-)}  
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_{1} - k_3)^2}{p^+} \bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_3)^2}
\frac{1}{(k_1^- + k_3^-)(p^--k_1^- - k_3^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad \bigg(4\frac{({\bm{k}}_{1}+ {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_1 - k_3)^2}{p^+} \bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_3}T^{b_1}T^{b_2})
&&\bigg[ \frac{2p^+}{(p - k_1)^2}
\bigg( 
\frac{6}{-k_1^- - k_3^-} - \frac{3}{p^- - k_1^- - k_3^-}
\bigg) 
+
 \frac{2p^+}{(p - k_3)^2}
\bigg(
 \frac{6}{k_1^- + k_3^-} + \frac{3}{-p^-}
\bigg)
\notag \\
&&& +
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(p^- - k_1^- - k_3^-)(k_{1}^- + k_3^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad 
 \bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_1 - k_3)^2}{p^+}  
\bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_3)^2}
\frac{1}{(k_{1}^- + k_3^-)(-p^-)} 
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_{1} - k_3)^2}{p^+} \bigg)
\bigg]
\end{align}
and
\begin{align}
  \label{eq:78}
(3I23) =&
   \frac{ g^4  {\bm{q}}^2}{p^2(p-k_2 - k_3)^2} &&\bigg\{
\notag \\
&\tr(T^{a}T^{b_2}T^{b_3}T^{b_1})
&&\bigg[ \frac{2p^+}{(p - k_2)^2}
\bigg(
\frac{6}{k_2^- + k_3^-} + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p - k_3)^2}
 \bigg(
 \frac{6}{-k_2^- - k_3^-} - \frac{3}{p^- - k_2^- - k_3^-}\bigg)
\notag \\
&&&
+
 \frac{2p^+}{(p - k_2)^2}
 \frac{1}{(-p^- )(k_2^- + k_3^-)}  
\bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_{2} - k_3)^2}{p^+} \bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_3)^2}
\frac{1}{(k_2^- + k_3^-)(p^--k_2^- - k_3^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad \bigg(4\frac{({\bm{k}}_{2}+ {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_2 - k_3)^2}{p^+} \bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_3}T^{b_2}T^{b_1})
&&\bigg[ \frac{2p^+}{(p - k_2)^2}
\bigg( 
\frac{6}{-k_2^- - k_3^-} - \frac{3}{p^- - k_2^- - k_3^-}
\bigg) 
+
 \frac{2p^+}{(p - k_3)^2}
\bigg(
 \frac{6}{k_2^- + k_3^-} + \frac{3}{-p^-}
\bigg)
\notag \\
&&& +
 \frac{2p^+}{(p - k_2)^2}
 \frac{1}{(p^- - k_2^- - k_3^-)(k_{2}^- + k_3^-)} 
\notag \\
&&&
\qquad \qquad \qquad \qquad \qquad \qquad 
 \bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_2 - k_3)^2}{p^+}  
\bigg)
\notag \\
&&&+
 \frac{2p^+}{(p - k_3)^2}
\frac{1}{(k_{2}^- + k_3^-)(-p^-)} 
\bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-k_{2} - k_3)^2}{p^+} \bigg)
\bigg]
\end{align}

\subsubsection{Diagram 4I2}
Here we need the induced vertex of the 3rd order given by
\begin{align}
  \label{eq:42}
&\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 )
=
g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[
\frac{f^{b_3b_1e_2}f^{e_2c_1e_1}f^{c_2e_1a}}{(-k_3^-)(-k_2^-)(p-k_2)^-}
+
\frac{f^{b_3b_1e_2}f^{e_2c_2e_1}f^{c_1e_1a}}{(-k_3^-)(-k_2^-)(-p^-)}
\notag \\
+&
\frac{f^{b_3c_1e_2}f^{e_2c_2e_1}f^{b_1e_1a}}{(-k_3^-)(p-k_1-k_2)^-(-k_1)^-}
+
\frac{f^{b_3c_1e_2}f^{e_2b_1e_1}f^{c_2e_1a}}{(-k_3^-)(p-k_1-k_2)^-(p-k_2)^-}
\notag \\
+&
\frac{f^{b_3c_2e_2}f^{e_2c_1e_1}f^{b_1e_1a}}{(-k_3^-)(-p-k_1)^-(-k_1)^-}
+
\frac{f^{b_3c_2e_2}f^{e_2b_1e_1}f^{c_1e_1a}}{(-k_3^-)(-p-k_1)^-(-p)^-}
\bigg]
\end{align}
which needs to be contracted with
\begin{align}
  \label{eq:43}
-gf^{c_1b_2c_2}{\Gamma}_{+}^{\mu\nu} (p,r) =&-gf^{c_1b_2c_2}\big[ g^{\mu\nu} 2p^+ - (n^+)^\mu( r +  2k_2)^\nu  -
( p -  2k_2)^\mu (n^+)^\nu 
\notag \\
&
+ \frac{{\bm{k}}_2^2}{p^+} (n^+)^\mu (n^+)^\nu\big]
\end{align}
where $r = p - k_2$. This time I consider first the color algebra part i.e.
\begin{align}
  \label{eq:44}
&f^{c_1b_2c_2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) = g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[
\frac{f^{b_3b_1e_2}f^{e_2c_1e_1} f^{c_1b_2c_2}  f^{c_2e_1a}}{(-k_3^-)(-k_2^-)(p-k_2)^-}
+
\frac{f^{b_3b_1e_2}f^{e_2c_2e_1} f^{c_1b_2c_2} f^{c_1e_1a}}{(-k_3^-)(-k_2^-)(-p^-)}
\notag \\
+&
\frac{f^{b_3c_1e_2} f^{c_1b_2c_2}  f^{e_2c_2e_1}f^{b_1e_1a}}{(-k_3^-)(p-k_1-k_2)^-(-k_1)^-}
+
\frac{f^{b_3c_1e_2} f^{c_1b_2c_2} f^{e_2b_1e_1}f^{c_2e_1a}}{(-k_3^-)(p-k_1-k_2)^-(p-k_2)^-}
\notag \\
+&
\frac{f^{b_3c_2e_2} f^{c_1b_2c_2} f^{e_2c_1e_1}f^{b_1e_1a}}{(-k_3^-)(-p-k_1)^-(-k_1)^-}
+
\frac{f^{b_3c_2e_2} f^{c_1b_2c_2} f^{e_2b_1e_1}f^{c_1e_1a}}{(-k_3^-)(-p-k_1)^-(-p)^-}
\bigg]
\notag \\
& 
=   %% erstes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[
\frac{f^{e_1ac_2}f^{c_2b_2c_1} f^{c_1e_2e_1}  f^{b_3b_1 e_2}}{(-k_3^-)(-k_2^-)(p-k_2)^-} %% Jacobi
-
\frac{f^{e_1ac_1}f^{c_1b_2c_2} f^{c_2e_2e_1} f^{b_3b_1e_2}}{(-k_3^-)(-k_2^-)(-p^-)}
\notag \\ %% Jacobi
+&
\frac{f^{ab_1 e_1} f^{c_2e_1e_2}  f^{e_2b_3c_1}f^{c_1b_2c_2}}{(-k_3^-)(p-k_1-k_2)^-(-k_1)^-} %%Jacobi
+
\frac{f^{e_1ac_2} f^{c_2b_2c_1} f^{c_1b_3e_2}f^{e_2b_1e_1}}{(-k_3^-)(p-k_1-k_2)^-(p-k_2)^-}
\notag \\
-&
\frac{f^{ab_1e_1} f^{c_1e_1e_2} f^{e_2b_3c_2}f^{c_2b_2c_1}}{(-k_3^-)(-p-k_1)^-(-k_1)^-} %%Jacobi
-
\frac{f^{e_1ac_1} f^{c_1b_2c_2} f^{c_2b_3e_2}f^{e_2b_1e_1}}{(-k_3^-)(-p-k_1)^-(-p)^-}
\bigg]
\end{align}
Make now use of the Jacobi-identity
\begin{align}
  \label{eq:45}
f^{abe}f^{ced} = -f^{ace}f^{bde} + f^{ade}f^{bce} = f^{cae}f^{ebd} - f^{cbe}f^{ead}
\end{align}
and rewrite the structure constants as
\begin{align}
  \label{eq:46}
&f^{c_1b_2c_2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) = %% erstes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[
\frac{f^{e_1ac_2}f^{c_2b_2c_1} f^{c_1b_3e_2}  f^{e_2b_1 e_1}   -   f^{e_1ac_2}f^{c_2b_2c_1} f^{c_1b_1e_2}  f^{e_2b_3 e_1} }{(-k_3^-)(-k_2^-)(p-k_2)^-} %% Jacobi
\notag \\
&-
\frac{f^{e_1ac_1}f^{c_1b_2c_2} f^{c_2b_3e_2} f^{e_2b_1e_1} - f^{e_1ac_1}f^{c_1b_2c_2} f^{c_2b_1e_2} f^{e_2b_3e_1} }{(-k_3^-)(-k_2^-)(-p^-)}
\notag \\ %% Jacobi
+&
\frac{f^{ c_2 a e_1} f^{e_1 b_1e_2}  f^{e_2b_3c_1}f^{c_1b_2c_2}  - f^{ c_2 b_1 e_1} f^{e_1 ae_2}  f^{e_2b_3c_1}f^{c_1b_2c_2}}{(-k_3^-)(p-k_1-k_2)^-(-k_1)^-} %%Jacobi
+
\frac{f^{e_1ac_2} f^{c_2b_2c_1} f^{c_1b_3e_2}f^{e_2b_1e_1}}{(-k_3^-)(p-k_1-k_2)^-(p-k_2)^-}
\notag \\
-&
\frac{f^{c_1 a e_1} f^{e_1b_1e_2} f^{e_2b_3c_2}f^{c_2b_2c_1} - f^{c_1 b_1 e_1} f^{e_1a e_2} f^{e_2b_3c_2}f^{c_2b_2c_1}}{(-k_3^-)(-p-k_1)^-(-k_1)^-} %%Jacobi
-
\frac{f^{e_1ac_1} f^{c_1b_2c_2} f^{c_2b_3e_2}f^{e_2b_1e_1}}{(-k_3^-)(-p-k_1)^-(-p)^-}
\bigg]
\end{align}
Next I use adjoint generator notation where $T^{b}_{ac} = if^{abc}$ which leads to
\begin{align}
  \label{eq:47}
&f^{c_1b_2c_2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) = %% erstes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[
\frac{\tr(T^aT^{b_2} T^{b_3}T^{b_1})   -   \tr(T^{a}T^{b_2} T^{b_1}T^{b_3}) }{(-k_3^-)(-k_2^-)(p-k_2)^-} %% Jacobi
\notag \\
&-
\frac{\tr(T^{a}T^{b_2}T^{b_3}T^{b_1}) -\tr(T^{a}T^{b_2}T^{b_3}T^{b_1})  }{(-k_3^-)(-k_2^-)(-p^-)}
\notag \\ %% Jacobi
+&
\frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  - \tr(T^{a}T^{b_3}T^{b_2}T^{b_1}) }{(-k_3^-)(p-k_1-k_2)^-(-k_1)^-} %%Jacobi
+
\frac{\tr(T^{a}T^{b_2}T^{b_3}T^{b_1})  }{(-k_3^-)(p-k_1-k_2)^-(p-k_2)^-}
\notag \\
-&
\frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})   - \tr(T^{a}T^{b_3}T^{b_2}T^{b_1}) }{(-k_3^-)(-p-k_1)^-(-k_1)^-} %%Jacobi
-
\frac{\tr(T^{a}T^{b_2}T^{b_3}T^{b_1})  }{(-k_3^-)(-p-k_1)^-(-p)^-}
\bigg]. 
\end{align}
Next I group momentum structure following the color structure. Note that $\tr( T^{a} T^{b} T^{c} T^{d}) = \tr(  T^{d} T^{c} T^{b} T^{a})$. We find:
\begin{align}
  \label{eq:48}
&f^{c_1b_2c_2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) = %% erstes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) \frac{1}{-k_3^-}
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\notag \\
&+
 \frac{1}{(p-k_1-k_2)^- (-k_1^-)} + \frac{1}{(p-k_1-k_2)^- (p-k_2)^-} 
-
 \frac{1}{(-p-k_1)^- (-k_1^-)} -  \frac{1}{(-p-k_1)^-(-p^-)}
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) \frac{1}{-k_3^-} 
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) \frac{1}{-k_3^-} 
\bigg(
 \frac{1}{(p-k_1-k_2)^- (-k_1^-)} - \frac{1}{(-p-k_1)^- (-k_1^-)}
\bigg)
\bigg]
\notag \\
&= %%zweites ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) \frac{1}{-k_3^-}
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\notag \\
&+
 \frac{1}{(p-k_2)^- (-k_1^-)}  
-
 \frac{1}{(-p^-) (-k_1^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) \frac{1}{-k_3^-} 
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) \frac{1}{-k_3^-} 
\bigg(
 \frac{1}{(p-k_1-k_2)^- (-k_1^-)} - \frac{1}{(-p-k_1)^- (-k_1^-)}
\bigg)\bigg]
\end{align}
with
\begin{align}
  \label{eq:49}
{\Gamma}_{+}^{--} (p,r) =- 4 p^-  +  2k_2^-   + 4\frac{{\bm{k}}_2^2}{p^+}  
=
-4(p^- - k_2^-) - 2k_2^-  + 4\frac{{\bm{k}}_2^2}{p^+}  
\end{align}
we obtain, where the factor $1/2$ in front is a symmetry-factor
\begin{align}
  \label{eq:50}
(4I2) =& \frac{1}{2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) \frac{-i}{p^2}
\frac{-i}{(p-k_2)^2} [-gf^{c_1b_2c_2}{\Gamma}_{+}^{\mu\nu} (p,r)]
\notag \\
=& %% erstes ==
- 4g^4 {\bm{q}}^2  \frac{p^2}{(p-k^2)^2} \bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) \frac{1}{-k_3^-}
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\notag \\
&+
 \frac{1}{(p-k_2)^- (-k_1^-)}  
-
 \frac{1}{(-p^-) (-k_1^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) \frac{1}{-k_3^-} 
\bigg(
\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) \frac{1}{-k_3^-} 
\bigg(
 \frac{1}{(p-k_1-k_2)^- (-k_1^-)} - \frac{1}{(-p-k_1)^- (-k_1^-)}
\bigg)\bigg]
\notag \\
&
\bigg[-2p^- + k_2^-  + 2\frac{{\bm{k}}_2^2}{p^+} \bigg]
\end{align}
The following simplifications occur:
\begin{align}
  \label{eq:51}
\bigg(
&\frac{1}{(-k_2^-)(p-k_2)^-} - \frac{1}{(-k_2^-)(-p^-)} 
+
 \frac{1}{(p-k_2)^- (-k_1^-)}  
-
 \frac{1}{(-p^-) (-k_1^-)} 
\bigg) \bigg[2p^- - k_2^-  \bigg] 
\notag \\
=&
\bigg(
 \frac{2}{(-k_2^-) } +  \frac{1}{(p-k_2)^-} + \frac{2}{(-k_2^-)}  + \frac{1}{(-p^-)} 
+
 \frac{2}{ (-k_1^-)}  + \frac{-k_2^-}{(p-k_2)^- (-k_1^-)}  
\notag \\ 
& +\frac{2}{ (-k_1^-)} +  \frac{-k_2^-}{(-p^-) (-k_1^-)} 
\bigg)
\notag \\
& =\frac{4}{(-k_2^-) } + \frac{4}{(-k_1-) } + \bigg( \frac{1}{(p-k_2)^-} + \frac{1}{-p^-} \bigg)\frac{-k_1^- - k_2^-}{k_1^-}
\end{align}
It might be more convenient to restrict to a certain parametrization of the minus components of the momenta. The natural choice seems to be $p^-$ $k_1^-$, $k_3^-$ while $k_2^- = -k_1^- - k_3^-$. Eq.(\ref{eq:48}) then becomes
\begin{align}
  \label{eq:52}
&f^{c_1b_2c_2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) = %% erstes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) \frac{1}{-k_3^-}
\bigg(
\frac{1}{(k_1^- + k_3^-)(p+ k_1^- + k_3^- )^-} - \frac{1}{(k_1^- + k_3^-)(-p^-)} 
\notag \\
&+
 \frac{1}{(p+ k_3)^- (-k_1^-)} + \frac{1}{(p+k_3)^- (p+ k_1 + k_3)^-} 
-
 \frac{1}{(-p-k_1)^- (-k_1^-)} -  \frac{1}{(-p-k_1)^-(-p^-)}
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) \frac{1}{-k_3^-} 
\bigg(
\frac{1}{(k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{(k_1^- +k_3^-)(-p^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) \frac{1}{-k_3^-} 
\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)} - \frac{1}{(-p-k_1)^- (-k_1^-)}
\bigg)
\bigg]
\notag \\
&= %%zweites ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) \frac{1}{-k_3^-}
\bigg(
\frac{1}{(k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{(k_1^- + k_3^-)(-p^-)} 
\notag \\
&+
 \frac{1}{(p+k_1 + k_3)^- (-k_1^-)}  
-
 \frac{1}{(-p^-) (-k_1^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) \frac{1}{-k_3^-} 
\bigg(
\frac{1}{(k_1^- + k_3^- )(p+k_1 + k_3)^-} - \frac{1}{(k_1^- + k_3^- )(-p^-)} 
\bigg)
\notag \\
&-
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) \frac{1}{-k_3^-} 
\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)} - \frac{1}{(-p-k_1)^- (-k_1^-)}
\bigg)\bigg]
\notag \\
&= %%drittes ==
 g^3 {\bm{q}}^2 (n^-)^\mu (n^-)^\nu 4 
\notag \\
&
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) 
\bigg(
\frac{1}{k_1^- (k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{k_1^-(k_1^- + k_3^-)(-p^-)} \bigg)
\notag \\
&+
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) 
\bigg(
\frac{1}{k_3^-(k_1^- + k_3^- )(p+k_1 + k_3)^-} - \frac{1}{k_3^-(k_1^- + k_3^- )(-p^-)} 
\bigg)
\notag \\
&+
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) 
\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)k_3^-} - \frac{1}{(-p-k_1)^- (-k_1^-)k_3^-}
\bigg)\bigg]
\end{align}
and (\ref{eq:49})
\begin{align}
  \label{eq:53}
{\Gamma}_{+}^{--} (p,r) =&- 4 p^-  -  2(k_1^- + k_3^-)   + 4\frac{{\bm{k}}_2^2}{p^+}  
=
-4(p^- + k_1^- + k_3^-) + 2(k_1^- + k_3^-)  + 4\frac{{\bm{k}}_2^2}{p^+}  
\notag \\
&=
-4(p^- + k_3^-) - 2k_1^- + 2k_3^-  + 4\frac{{\bm{k}}_2^2}{p^+}  
= 4(-p^- - k_1^-) + 2k_1^- - 2k_3^- + 4\frac{{\bm{k}}_2^2}{p^+}  
\end{align}
and the expression to be considered reads then as
\begin{align}
  \label{eq:54}
(4I2) =& \frac{1}{2}\Delta^{c_1c_2b_1b_3}(-p,p-k_2,-k_1, -k_3 ) \frac{-i}{p^2}\frac{-i}{(p-k_2)^2} [-gf^{c_1b_2c_2}{\Gamma}_{+}^{\mu\nu} (p,r)]
\notag \\
=&
 2g^4 {\bm{q}}^2  \frac{1}{p^2(p-k_2)^2} 
\bigg[\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) %%a231
\bigg(
\frac{1}{k_1^- (k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{k_1^-(k_1^- + k_3^-)(-p^-)} \bigg)
\notag \\
&+
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) %%a213
\bigg(
\frac{1}{k_3^-(k_1^- + k_3^- )(p+k_1 + k_3)^-} - \frac{1}{k_3^-(k_1^- + k_3^- )(-p^-)} 
\bigg)
\notag \\
&+
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) %%a321
\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)k_3^-} - \frac{1}{(-p-k_1)^- (-k_1^-)k_3^-}
\bigg)\bigg]
\Gamma^{--}_+(p,p -k_2)
\end{align}
The following simplifications are then possible
\begin{align}
  \label{eq:55}
&
\bigg(
\frac{1}{k_1^- (k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{k_1^-(k_1^- + k_3^-)(-p^-)} \bigg)
 (-4p^- - 2(k_1 + k_3)^-)
\notag \\
&=
\frac{-4}{k_1^-(k_1^- + k_3^-)} + \frac{2}{k_1^-(p^- + k_1^- + k_3^-)}
+ \frac{-4}{k_1^-(k_1^- + k_3^-)} + \frac{2}{k_1^-(-p^-)}
\notag \\
&=
\frac{-8}{k_1^-(k_1^- + k_3^-)} + \frac{2}{k_1^-(p^- + k_1^- + k_3^-)}+ \frac{2}{k_1^-(-p^-)}
\end{align}
and 
\begin{align}
  \label{eq:56}
&\bigg(
\frac{1}{k_3^-(k_1^- + k_3^- )(p+k_1 + k_3)^-} - \frac{1}{k_3^-(k_1^- + k_3^- )(-p^-)} 
\bigg)  (-4p^- - 2(k_1 + k_3)^-)
\notag \\
&=\frac{-4}{k_3^-(k_1^- + k_3^-)} + \frac{2}{k_3^-(p^- + k_1^- + k_3^-)}
+\frac{-4}{k_3^-(k_1^- + k_3^-)} + \frac{2}{k_3^-(-p^-)}
\notag \\
&
=\frac{-8}{k_3^-(k_1^- + k_3^-)} + \frac{2}{k_3^-(p^- + k_1^- + k_3^-)} + \frac{2}{k_3^-(-p^-)}
\end{align}
and finally
\begin{align}
  \label{eq:57}
&\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)k_3^-} - \frac{1}{(-p-k_1)^- (-k_1^-)k_3^-}
\bigg)  ( -4(p^-+k_3^-) - 2k_1^- +2 k_3^-)
\notag \\
&= \frac{-4}{-k_1^-k_3^-} + \frac{2}{(p^-+ k_3^-)k_3^-} + \frac{2}{(p^- + k_3^-)(-k_1^-)} 
\notag \\
&
+  \frac{-4}{-k_1^-k_3^-}  + \frac{2}{(-p^- - k_1^-)k_3^-} + \frac{2}{(-p^- - k_1^-)(-k_1^-)}
\notag \\
&=
 \frac{-8}{-k_1^-k_3^-} + \frac{2}{(p^-+k_3^-)k_3^-} + \frac{2}{(p^- + k_3^-)(-k_1^-)}
\notag \\
& \qquad
 + \frac{2}{(-p^- - k_1^-)k_3^-} + \frac{2}{(-p^- - k_1^-)(-k_1^-)}
\end{align}
which gives
\begin{align}
  \label{eq:58}
(4I2) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p-q - k_1 - k_3)^2} \bigg\{\notag \\
&
\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) %%a231
\bigg(
\frac{-8}{k_1^-(k_1^- + k_3^-)} + \frac{2}{k_1^-(p^- + k_1^- + k_3^-)}+ \frac{2}{k_1^-(-p^-)}
\bigg) \notag \\
&
+\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) %%a213
\bigg(
\frac{-8}{k_3^-(k_1^- + k_3^-)} + \frac{2}{k_3^-(p^- + k_1^- + k_3^-)} + \frac{2}{k_3^-(-p^-)}
\bigg)
\notag \\
& +
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) %%a321
\bigg(
\frac{-8}{-k_1^-k_3^-} + \frac{2}{(p^-+k_3^-)k_3^-} +
  \frac{2}{(-p^- - k_1^-)k_3^-}
\notag \\
& + \frac{2}{(p^- + k_3^-)(-k_1^-)}  + \frac{2}{(-p^- - k_1^-)(-k_1^-)}
\bigg)
\notag \\
&+\bigg[
\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) %%a231
\bigg(
\frac{1}{k_1^- (k_1^- + k_3^-)(p+k_1 + k_3)^-} - \frac{1}{k_1^-(k_1^- + k_3^-)(-p^-)} \bigg)
\notag \\
&+
\tr( T^{a} T^{b_2} T^{b_1} T^{b_3}) %%a213
\bigg(
\frac{1}{k_3^-(k_1^- + k_3^- )(p+k_1 + k_3)^-} - \frac{1}{k_3^-(k_1^- + k_3^- )(-p^-)} 
\bigg)
\notag \\
&+
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) %%a321
\bigg(
 \frac{1}{(p+k_3)^- (-k_1^-)k_3^-} - \frac{1}{(-p-k_1)^- (-k_1^-)k_3^-}
\bigg)\bigg]
 4\frac{{\bm{k}}_2^2}{p^+}  \bigg\}
\end{align}

\subsubsection{Diagram 4I1 and 4I3}
By exchanging indices we obtain
\begin{align}
  \label{eq:66}
(4I1) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p-q - k_2 - k_3)^2} \bigg\{\notag \\
&
\tr( T^{a} T^{b_1} T^{b_3} T^{b_2}) %%a231
\bigg(
\frac{-8}{k_2^-(k_2^- + k_3^-)} + \frac{2}{k_2^-(p^- + k_2^- + k_3^-)}+ \frac{2}{k_2^-(-p^-)}
\bigg) \notag \\
&
+\tr( T^{a} T^{b_1} T^{b_2} T^{b_3}) %%a213
\bigg(
\frac{-8}{k_3^-(k_2^- + k_3^-)} + \frac{2}{k_3^-(p^- + k_2^- + k_3^-)} + \frac{2}{k_3^-(-p^-)}
\bigg)
\notag \\
& +
\tr( T^{a} T^{b_3} T^{b_1} T^{b_2}) %%a321
\bigg(
\frac{-8}{-k_2^-k_3^-} + \frac{2}{(p^-+k_3^-)k_3^-} +
  \frac{2}{(-p^- - k_2^-)k_3^-}
\notag \\
& + \frac{2}{(p^- + k_3^-)(-k_2^-)}  + \frac{2}{(-p^- - k_2^-)(-k_2^-)}
\bigg)
\notag \\
&+
\bigg[
\tr( T^{a} T^{b_1} T^{b_3} T^{b_2}) %%a231
\bigg(
\frac{1}{k_2^- (k_2^- + k_3^-)(p+k_2 + k_3)^-} - \frac{1}{k_2^-(k_2^- + k_3^-)(-p^-)} \bigg)
\notag \\
&+
\tr( T^{a} T^{b_1} T^{b_2} T^{b_3}) %%a213
\bigg(
\frac{1}{k_3^-(k_2^- + k_3^- )(p+k_2 + k_3)^-} - \frac{1}{k_3^-(k_2^- + k_3^- )(-p^-)} 
\bigg)
\notag \\
&+
\tr( T^{a} T^{b_3} T^{b_1} T^{b_2}) %%a321
\bigg(
 \frac{1}{(p+k_3)^- (-k_2^-)k_3^-} - \frac{1}{(-p-k_2)^- (-k_2^-)k_3^-}
\bigg)\bigg]
 4\frac{{\bm{k}}_1^2}{p^+}  \bigg\}
\end{align}
and
\begin{align}
  \label{eq:67}
(4I3) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p-q - k_1 - k_2)^2} \bigg\{\notag \\
&
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) %%a231
\bigg(
\frac{-8}{k_1^-(k_1^- + k_2^-)} + \frac{2}{k_1^-(p^- + k_1^- + k_2^-)}+ \frac{2}{k_1^-(-p^-)}
\bigg) \notag \\
&
+\tr( T^{a} T^{b_3} T^{b_1} T^{b_2}) %%a213
\bigg(
\frac{-8}{k_2^-(k_1^- + k_2^-)} + \frac{2}{k_2^-(p^- + k_1^- + k_2^-)} + \frac{2}{k_2^-(-p^-)}
\bigg)
\notag \\
& +
\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) %%a321
\bigg(
\frac{-8}{-k_1^-k_2^-} + \frac{2}{(p^-+k_2^-)k_2^-} +
  \frac{2}{(-p^- - k_1^-)k_2^-}
\notag \\
& + \frac{2}{(p^- + k_2^-)(-k_1^-)}  +\frac{2}{(-p^- - k_1^-)(-k_1^-)}
\bigg)
\notag \\
&+
\bigg[
\tr( T^{a} T^{b_3} T^{b_2} T^{b_1}) %%a231
\bigg(
\frac{1}{k_1^- (k_1^- + k_2^-)(p+k_1 + k_2)^-} - \frac{1}{k_1^-(k_1^- + k_2^-)(-p^-)} \bigg)
\notag \\
&+
\tr( T^{a} T^{b_3} T^{b_1} T^{b_2}) %%a213
\bigg(
\frac{1}{k_2^-(k_1^- + k_2^- )(p+k_1 + k_2)^-} - \frac{1}{k_2^-(k_1^- + k_2^- )(-p^-)} 
\bigg)
\notag \\
&+
\tr( T^{a} T^{b_2} T^{b_3} T^{b_1}) %%a321
\bigg(
 \frac{1}{(p+k_2)^- (-k_1^-)k_2^-} - \frac{1}{(-p-k_1)^- (-k_1^-)k_2^-}
\bigg)\bigg]
 4\frac{{\bm{k}}_3^2}{p^+}  \bigg\}
\end{align}

\subsubsection{Diagram GH123a - ghost-diagrams}
We have 
\begin{align}
  \label{eq:59}
GH123a =& -(-g)^4 f^{c_1ac_2}f^{c_2b_3c_3}f^{c_3b_2c_4}f^{c_4b_1c_1} p^-(p^+)^3 \frac{i^4}{p^2(p-q)^2(p-k_1 - k_2)^2 (p-k_1)^2}
\notag \\
=&
-g^4\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-k_1 - k_2)^2 (p-k_1)^2}
\end{align}
and
\begin{align}
  \label{eq:60}
GH123b =&
-(-g)^4f^{c_2ac_1}f^{c_1b_1c_3}f^{c_3b_2c_4}f^{c_4b_3c_2} p^-(p^+)^3 \frac{i^4}{p^2(p-q+k_1 + k_2)^2 (p-q + k_1)^2 (p-q)^2}
\notag \\
=&
-g^4\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \frac{p^-(p^+)^3}{p^2 (p-q + k_1 + k_2)^2 (p-q + k_1)^2  (p-q)^2}
\end{align}
other diagrams can be obtained by corresponding permutations.


\subsubsection{Diagram GH132a and GH132b}
We obtain by interchanging indices
\begin{align}
  \label{eq:65}
GH132a =& -g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-k_1 - k_3)^2 (p-k_1)^2}
\end{align}
and
\begin{align}
  \label{eq:68}
GH132b =&
-g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  \frac{p^-(p^+)^3}{p^2(p-k_2)^2 (p-q + k_1)  (p-q)^2}
\end{align}


\subsubsection{Diagrams GH213a and GH213b}

\begin{align}
  \label{eq:69}
GH213a =& -g^4\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-k_1 - k_2)^2 (p-k_2)^2}
\end{align}
and
\begin{align}
  \label{eq:70}
GH231b =&
-g^4\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  \frac{p^-(p^+)^3}{p^2 (p-q +k_1 + k_2)^2 (p-q + k_2) (p-q)^2 }
\end{align}


\subsection{A list of all diagrams}
\label{sec:list}

We shall give in the following a list of all expression obtained up to now. We will state results with a minimal basis of color tensors which we chose to be $\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})$,  $\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})$ and $\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})$. We have
\begin{align}
  \label{eq:71}
 (4RRP) =& g^4  \bigg[
 \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{p^2(p - k_1)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
+ 
 \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{p^2(p - q+ k_1)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } \notag \\
&+ 
\frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
+ 
 \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
\notag \\
&+
\frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - k_1)^2 (p- q + k_2)^2 (p-q)^2 } 
+  
\frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - q+ k_1)^2 (p-  k_2)^2 (p-q)^2 }
\bigg]
\notag \\
& (p^+)^2 \bigg[ 
17 p^+p^- +  (p^2 + (p-q)^2)
 - 32 {\bm{q}}^2  + 8\frac{{\bm{q}}^4}{p^+p^-} + 6 \frac{{\bm{q}}^2}{p^+p^-} (p^2 + (p-q)^2)  
\bigg]
\end{align}
\begin{align}
  \label{eq:72}
(4G+12) =&
-g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) }{p^2 (p-k_1)^2 (p - k_1-k_2)^2}
 +
 \frac{\tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) }{p^2 (p-k_2)^2 (p - k_1-k_2)^2}
\big]
 \\
\label{eq:73}
 (4G+13) =& -g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) }{p^2 (p-k_1)^2 (p - q + k_2)^2}
 +
 \frac{\tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) }{p^2 (p-q + k_1 + k_2)^2 (p - q +k_2)^2}
\big] \\
\label{eq:74}
(4G+23) =&
-g^4 18(p^+)^2 \big[
 \frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) }{p^2 (p-k_2)^2 (p - q + k_1)^2}
 +
 \frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) }{p^2 (p-q + k_1 + k_2)^2 (p - q + k_1)^2}
\big]
\end{align}
\begin{align}
  \label{eq:75}
(3I12) =& g^4\frac{  {\bm{q}}^2}{p^2(p-k_1 - k_2)^2}
  \bigg\{
\notag \\
& \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\bigg[
 \frac{4p^+}{(p - k_1)^2}
 \frac{1}{(-p^- )(k_1^- + k_2^-)}  
\bigg(2\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  \frac{p^2  + (p-k_{1} - k_2)^2}{p^+} \bigg)
\notag \\
&+
 \frac{4p^+}{(p - k_2)^2}
\frac{1}{(k_1^- + k_2^-)(p^--k_1^- - k_2^-)} 
%\notag \\
%&
%\qquad \qquad \qquad \qquad \qquad \qquad 
\bigg(2\frac{({\bm{k}}_{1}+ {\bm{k}}_2)^2}{p^+}  +  \frac{p^2  + (p-k_1 - k_2)^2}{p^+} \bigg)
\notag \\
&+
 \frac{2p^+}{(p - k_1)^2}
\bigg(
\frac{6}{k_1^- + k_2^-} + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p - k_2)^2}
 \bigg(
 \frac{6}{-k_1^- - k_2^-} - \frac{3}{p^- - k_1^- - k_2^-}\bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\bigg[
  \frac{2p^+}{(p - k_2)^2}
\frac{1}{(k_{1}^- + k_2^-)(-p^-)} 
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_{1} - k_2)^2}{p^+} \bigg)
\notag \\
&+
\frac{2p^+}{(p - k_1)^2}
 \frac{1}{(p^- - k_1^- - k_2^-)(k_{1}^- + k_2^-)} 
%\notag \\
%&
%
 \bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_2)^2}{p^+}  +  2\frac{p^2  + (p-k_1 - k_2)^2}{p^+}  
\bigg)
\notag \\
&+
 \frac{2p^+}{(p - k_1)^2}
\bigg( 
\frac{6}{-k_1^- - k_2^-} - \frac{3}{p^- - k_1^- - k_2^-}
\bigg) 
+
 \frac{2p^+}{(p - k_2)^2}
\bigg(
 \frac{6}{k_1^- + k_2^-} + \frac{3}{-p^-}
\bigg)
\bigg] \bigg\}
\notag \\
\end{align}
\begin{align}
  \label{eq:79}
(3I13) =&
   g^4 \frac{  {\bm{q}}^2}{p^2(p- q + k_2 )^2} \bigg\{
\notag \\
&\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[ 
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(-p^- )(-k_2^- )}  
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q - k_{2} )^2}{p^+} \bigg)
\notag \\
&
+
 \frac{2p^+}{(p-  q + k_1 + k_2)^2}
\frac{1}{(- k_2^- )(p^- + k_2^- )} 
\bigg(4\frac{({\bm{k}}_{1}+ {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q + k_2 )^2}{p^+} \bigg)
\notag \\
&+
\frac{2p^+}{(p - k_1)^2}
\bigg(
\frac{6}{-k_2^- } + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p - q +k_1 + k_2)^2}
 \bigg(
 \frac{6}{k_2^-} - \frac{3}{p^- +  k_2^-}\bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\bigg[
%\notag \\
%&+
%\notag \\
%& +
 \frac{2p^+}{(p - k_1)^2}
 \frac{1}{(p^- +  k_2^- )( - k_{2}^- )} 
 \bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p- q + k_2 )^2}{p^+}  
\bigg)
\notag \\
&+
 \frac{2p^+}{(p - q + k_1 + k_2 )^2}
\frac{1}{(-k_{2}^- )(-p^-)} 
\bigg(4\frac{({\bm{k}}_{1} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q + k_{2})^2}{p^+} \bigg)
\notag \\
&+
 \frac{2p^+}{(p - k_1)^2}
\bigg( 
\frac{6}{  k_2^-} - \frac{3}{p^- + k_2^- }
\bigg) 
+
 \frac{2p^+}{(p -q +  k_1 + k_2)^2}
\bigg(
 \frac{6}{- k_2^- } + \frac{3}{-p^-}
\bigg)
\bigg] \bigg\}
\end{align}

\begin{align}
  \label{eq:80}
(3I23) =&
   g^4\frac{   {\bm{q}}^2}{p^2(p-q + k_1 )^2} \bigg\{
\notag \\
&\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
 \frac{2p^+}{(p - k_2)^2}
 \frac{1}{(-p^- )(-k_1^-)}  
\bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q + k_{1} )^2}{p^+} \bigg)
\notag \\
&+
 \frac{2p^+}{(p - q + k_1 +  k_2)^2}
\frac{1}{(-k_1^-)(p^- + k_1^- )} 
 \bigg(4\frac{({\bm{k}}_{2}+ {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q +k_1 )^2}{p^+} \bigg)
\notag \\
&+
 \frac{2p^+}{(p - k_2)^2}
\bigg(
\frac{6}{- k_1^- } + \frac{3}{-p^- }
\bigg)  + 
 \frac{2p^+}{(p -q +  k_1 + k_2)^2}
 \bigg(
 \frac{6}{ k_1^- } - \frac{3}{p^- + k_1^-}\bigg)
\bigg]
\notag \\
&\big[ %%neuer Generator
\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\bigg[
 \frac{2p^+}{(p -  k_2)^2}
 \frac{1}{(p^- + k_1^- )(- k_{1}^- )} 
 \bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p-q +k_1  )^2}{p^+}  
\bigg)
\notag \\
&+
 \frac{2p^+}{(p - q + k_1 + k_2 )^2}
\frac{1}{(- k_{1}^- )(-p^-)} 
\bigg(4\frac{({\bm{k}}_{2} + {\bm{k}}_3)^2}{p^+}  +  2\frac{p^2  + (p- q + k_{1} )^2}{p^+} \bigg)
\notag \\
&+
 \frac{2p^+}{(p - k_2)^2}
\bigg( 
\frac{6}{k_1^- } - \frac{3}{p^- +  k_1^-}
\bigg) 
+
 \frac{2p^+}{(p - q + k_1 + k_2)^2}
\bigg(
 \frac{6}{- k_1 } + \frac{3}{-p^-}
\bigg)
\bigg]\bigg\}
\end{align}
\begin{align}
  \label{eq:83}
(4I1) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p - k_1 )^2} 
\bigg\{
   \tr( T^{a} T^{b_1} T^{b_2} T^{b_3})
   \bigg[
        \frac{-8}{(-k_1^- - k_2^-)( - k_1^- )} +
        \frac{2}{(-k_1^- - k_2^-) (p^- - k_1^- )} 
\notag \\
        &+
        \frac{2}{(-k_1^- - k_2^-) (-p^-)} 
        + 4\frac{{\bm{k}}_1^2}{p^+} 
        \bigg(
             \frac{1}{(-k_1^- - k_2^-)(- k_1^- )(p -k_1 )^-} -
             \frac{1}{(-k_1^- - k_2^-)(-k_1^-)(-p^-)}   
        \bigg)     
   \bigg]
\notag \\   
   &+
   \tr( T^{a} T^{b_2} T^{b_1} T^{b_3})
   \bigg[
        \frac{-8}{- k_2^- (-k_1^- - k_2^-)} + 
        \frac{2}{(p^- - k_1^- - k_2^- )(-k_1^- - k_2^-)} 
\notag \\        
        &+
        \frac{2}{(-p^- - k_2^-)(-k_1^- - k_2^-)} + 
        \frac{2}{(p^- - k_1^- - k_2^-)(-k_2^-)}  +
        \frac{2}{(-p^- - k_2^-)(-k_2^-)}
\notag \\
         &+ 4\frac{{\bm{k}}_1^2}{p^+} 
         \bigg(
               \frac{1}{(p^-- k_1^- - k_2^-) (-k_2^-)(-k_1^- - k_2^-)} - 
               \frac{1}{(-p-k_2)^- (-k_2^-)(-k_1^- -k_2^-)}
         \bigg)
   \bigg]
\notag \\
   &+
   \tr( T^{a} T^{b_1} T^{b_3} T^{b_2})
   \bigg[
        \frac{-8}{k_2^-(-k_1 )} +
        \frac{2}{k_2^-(p^- -  k_1^- )} +
        \frac{2}{k_2^-(-p^-)} 
\notag \\        
        &+
        4\frac{{\bm{k}}_1^2}{p^+}
        \bigg(
              \frac{1}{k_2^- (- k_1^-)(p- k_1 )^-} - 
              \frac{1}{k_2^-(- k_1^-)(-p^-)}
        \bigg)
   \bigg]
\bigg\}
\end{align}
\begin{align}
  \label{eq:84}
(4I2) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p - k_2 )^2} 
\bigg\{
   \tr( T^{a} T^{b_1} T^{b_2} T^{b_3})
   \bigg[
        \frac{-8}{- k_1^- (-k_1^- - k_2^-)} + 
        \frac{2}{(p^- - k_1^- - k_2^- )(-k_1^- - k_2^-)} 
\notag \\        
        &+
        \frac{2}{(-p^- - k_1^-)(-k_1^- - k_2^-)} + 
        \frac{2}{(p^- - k_1^- - k_2^-)(-k_1^-)}  + 
        \frac{2}{(-p^- - k_1^-)(-k_1^-)}
\notag \\
         &+ 4\frac{{\bm{k}}_2^2}{p^+} 
         \bigg(
               \frac{1}{(p^-- k_1^- - k_2^-) (-k_1^-)(-k_1^- - k_2^-)} - 
               \frac{1}{(-p-k_1)^- (-k_1^-)(-k_1^- -k_2^-)}
         \bigg)
   \bigg]
\notag \\   
   &+
   \tr( T^{a} T^{b_2} T^{b_1} T^{b_3})
   \bigg[
        \frac{-8}{(-k_1^- - k_2^-)( - k_2^- )} +
        \frac{2}{(-k_1^- - k_2^-) (p^- - k_2^- )} 
\notag \\
        &+
        \frac{2}{(-k_1^- - k_2^-) (-p^-)} 
        + 4\frac{{\bm{k}}_2^2}{p^+} 
        \bigg(
             \frac{1}{(-k_1^- - k_2^-)(- k_2^- )(p -k_2 )^-} -
             \frac{1}{(-k_1^- - k_2^-)(-k_2^-)(-p^-)}   
        \bigg)     
   \bigg]
\notag \\
   &+
   \tr( T^{a} T^{b_1} T^{b_3} T^{b_2})
   \bigg[
        \frac{-8}{k_1^-(-k_2 )} +
        \frac{2}{k_1^-(p^- -  k_2^- )} +
        \frac{2}{k_1^-(-p^-)} 
\notag \\        
        &+
        4\frac{{\bm{k}}_2^2}{p^+}
        \bigg(
              \frac{1}{k_1^- (- k_2^-)(p- k_2 )^-} - 
              \frac{1}{k_1^-(- k_2^-)(-p^-)}
        \bigg)
   \bigg]
\bigg\}
\end{align}
\begin{align}
  \label{eq:85}
(4I3) =&  2g^4 {\bm{q}}^2  \frac{1}{p^2(p - q +k_1 + k_2 )^2} 
\bigg\{
   \tr( T^{a} T^{b_1} T^{b_2} T^{b_3})
   \bigg[
        \frac{-8}{(k_1^-)(  k_1^- + k_2^- )} +
        \frac{2}{(k_1^- ) (p^- + k_1^- + k_2^- )} 
\notag \\
        &+
        \frac{2}{(k_1^- ) (-p^-)} 
        + 4\frac{{\bm{k}}_3^2}{p^+} 
        \bigg(
             \frac{1}{(k_1^- )( k_1^- + k_2^- )(p^- +k_1^- + k_2^- )} -
             \frac{1}{(k_1^- )(-k_1^- - k_2^-)(-p^-)}   
        \bigg)     
   \bigg]
\notag \\   
   &+
  \tr( T^{a} T^{b_2} T^{b_1} T^{b_3})
   \bigg[
        \frac{-8}{k_2^-(k_1 + k_2^- )} +
        \frac{2}{k_2^-(p^- +  k_1^- +k_2^-)} +
        \frac{2}{k_2^-(-p^-)} 
\notag \\        
        &+
        4\frac{{\bm{k}}_3^2}{p^+}
        \bigg(
              \frac{1}{k_2^- ( k_1^-+k_2^-)(p^- + k_1^- +k_2^- )^-} - 
              \frac{1}{k_2^-( k_1^- + k_2^-)(-p^-)}
        \bigg)
   \bigg]
\notag \\
   &+
   \tr( T^{a} T^{b_1} T^{b_3} T^{b_2})
   \bigg[
        \frac{-8}{- k_1^- (k_2^- )} + 
        \frac{2}{(p^- + k_2^- )( k_2^-)} 
\notag \\        
        &+
        \frac{2}{(-p^- - k_1^-)(k_2^- )} + 
        \frac{2}{(p^- + k_2^-)(-k_1^-)}  + 
        \frac{2}{(-p^- - k_1^-)(-k_1^-)}
\notag \\
         &+ 4\frac{{\bm{k}}_3^2}{p^+} 
         \bigg(
               \frac{1}{(p^- + k_1^- ) (-k_2^-)(k_1^- )} - 
               \frac{1}{(-p-k_2)^- (-k_2^-)(k_1^-)}
         \bigg)
   \bigg]
\bigg\}
\end{align}
\begin{align}
  \label{eq:86}
GH123a =&
-g^4\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-k_1 - k_2)^2 (p-k_1)^2}
\\
  \label{eq:87}
GH123b =&-g^4\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \frac{p^-(p^+)^3}{p^2 (p -q + k_1 + k_2)^2 (p- q + k_1)^2(p-q)^2 }
\end{align}

\begin{align} 
  \label{eq:90}
GH213a =& -g^4\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-k_1 - k_2)^2 (p-k_2)^2}
\\
\label{eq:91}
GH213b =&
-g^4\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  \frac{p^-(p^+)^3}{p^2 (p-q +k_1 + k_2)^2 (p-q + k_2) (p-q)^2 }
\end{align}
\begin{align}
  \label{eq:88}
GH132a =& -g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  \frac{p^-(p^+)^3}{p^2(p-q)^2(p-q + k_2 )^2 (p-k_1)^2}
\\
\label{eq:89}
GH132b =&
-g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  \frac{p^-(p^+)^3}{p^2(p-k_2)^2 (p-q + k_1)  (p-q)^2}
\end{align}



\subsection{Intelligent combinations of diagrams}
\label{sec:combinations}

In the following we attempt to calculate the sum of all of the expressions listed above. In order to do so we restrict at first ourselves to the color structure $\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})$. With the remaining two structure we will deal with afterwards. We gather the summed diagrams in new contributions which we label by capital letters $A, B, C ....$. 

\subsubsection{$\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})$ contributions}
Using contributions from (4RRP), (4G+12), (4G+23), (GH123a) and (GH123b) (which exhausts (GHijkx) -diagrams) we find
\begin{align}
  \label{eq:92}
A_1 &= g^4 \frac{(p^+)^3p^-}{p^2 (p-k_1)^2 (p - k_1 - k_2)^2} (17 + 2 - 18 -1) = 0 \\
\label{eq:93}
A_2 &= g^4 \frac{(p^+)^3p^-}{(p-q)^2 (p -q+k_1)^2 (p-q + k_1 + k_2)^2 p^2} (17 + 2 - 18 -1) = 0.
\end{align}
Using contributions from (4RRP), (4G+12) and (4G+23) (which exhausts (4G+ij) diagrams)  we find
\begin{align}
  \label{eq:94}
B_1=& g^4\frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   (p^+)^2}{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} (-{\bm{p}}^2 - ({\bm{q }} - {\bm{p}})^2  - 32 {\bm{q}}^2 + 8 \frac{{\bm{q}}^4}{p^+p^-}+  18 ({\bm{q }} - {\bm{p}})^2 ) \notag \\
+&  g^4\frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) (p^+)^2}{p^2 (p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} (-{\bm{p}}^2 - ({\bm{q }} - {\bm{p}})^2    - 32 {\bm{q}}^2 + 8 \frac{{\bm{q}}^4}{p^+p^-}  + 18({\bm{q }} - {\bm{p}})^2 ).
\end{align}
Using contributions from (4RRP), (3I12) and (3I23)  (which exhausts the (4RPP) diagram) we find

\begin{align}
  \label{eq:95}
C_1 &= g^4 6\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \bigg[
\bigg(
\frac{p^+}{(p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} 
+
 \frac{p^+}{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 } 
\notag \\
&
+
\frac{p^+}{(p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
+
 \frac{p^+}{p^2 (p-q +k_1)^2 (p-q + k_1 + k_2)^2 }\bigg)
\frac{{\bm{q}}^2}{p^-} 
\notag \\
&+
  \frac{p^+}{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 } \frac{{\bm{q}}^2}{-p^- } %\notag \\
 %&
-
  \frac{p^+}{p^2 (p-k_2)^2 (p-k_1 - k_2)^2 } \frac{{\bm{q}}^2}{ p^- - k_1^- - k_2^- } \notag \\
&-
  \frac{p^+}{p^2 (p-k_2)^2 (p-q + k_1 )^2 } \frac{{\bm{q}}^2}{ p^- + k_1^- } +
  \frac{p^+}{p^2  (p-q + k_1 )^2 (p -q - k_1 + k_2)^2 } \frac{{\bm{q}}^2}{ -p^-  } \bigg]
\notag \\
&= %% zweites ==
 g^4 6\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) 
\bigg[
\bigg(
\frac{p^+}{(p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} 
\notag \\
&+
\frac{p^+}{(p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
+
\bigg)
\frac{{\bm{q}}^2}{p^-} 
\notag \\
&
-
  \frac{p^+}{p^2 (p-k_2)^2 (p-k_1 - k_2)^2 } \frac{{\bm{q}}^2}{ p^- - k_1^- - k_2^- } 
-
  \frac{p^+}{p^2 (p-k_2)^2 (p-q + k_1 )^2 } \frac{{\bm{q}}^2}{ p^- + k_1^- } \bigg]
\end{align}
Using now contributions from (3I12), (3I23), (4I1), (4I2) and (4I3) we find
\begin{align}
  \label{eq:81}
D_1 &= g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \bigg[ 
                      \frac{1}{-p^-(k_1^- + k_2^-)} \frac{1}{p^2(p-k_1)^2} +
                      \frac{1}{-p^-(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_1)^2} 
\notag \\
                      &+
                      \frac{1}{(p^- - k_1^- - k_2^-) (k_1^- + k_2^-)} \frac{1}{p^2(p-k_2)^2} +
                      \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_2)^2}
\notag \\ %% (3I12 vorbei) 3I23 beginnt
                     &+
                       \frac{1}{(p^- +k_1^-)(- k_1^- )} \frac{1}{p^2(p-k_2)^2} +
                      \frac{1}{(p^- +k_1^-)(-k_1^- )} \frac{1}{(p- q + k_1 )^2 (p-k_2)^2} 
\notag \\
                      &+
                      \frac{1}{(-p^- ) (-k_1^- )} \frac{1}{p^2(p-q + k_1 + k_2)^2} +
                      \frac{1}{(-p^-)(-k_1^- )} \frac{1}{(p- q + k_1 )^2 (p-q + k_1 + k_2)^2}
\notag \\ %%4I1 beginnt
                     &+ \frac{1}{(p^- -k_1^-)(- k_1^- - k_2^- )} \frac{1}{p^2(p-k_1)^2} 
                      +\frac{1}{(-p^- )(-k_1^- - k_2^- )} \frac{1}{p^2 (p-k_1)^2} 
\notag \\ %%4I2 beginnt
                      &+
                      \frac{1}{(p^- - k_1^- -k_2^- ) (-k_1^- - k_2^- )} \frac{1}{p^2(p- k_2)^2} 
                      + \frac{1}{(p^- - k_1^- - k_2^- ) (-k_1^- )} \frac{1}{p^2(p- k_2)^2} 
\notag \\
                      &+             
                      \frac{1}{(-p^- -k_1^-) (-k_1^- -k_2^- )} \frac{1}{p^2(p- k_2)^2} 
                      + \frac{1}{(-p^- -  k_1^- ) (-k_1^- )} \frac{1}{p^2(p- k_2)^2} 
\notag \\ %%4I3 beginnt                     
                      &+  
                      \frac{1}{(p^- + k_1^- + k_2^-)k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2} 
                      +\frac{1}{(-p^- )k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2}
\bigg]
\notag \\
 &=  %%zweites ==
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \bigg[ 
                      %\frac{1}{-p^-(k_1^- + k_2^-)} \frac{1}{p^2(p-k_1)^2} 
                      %+
                      \frac{1}{-p^-(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_1)^2} 
\notag \\
                      &
                      %+
                      %\frac{1}{(p^- - k_1^- - k_2^-) (k_1^- + k_2^-)} \frac{1}{p^2(p-k_2)^2} 
                      +
                      \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_2)^2}
%\notag \\ %% (3I12 vorbei) 3I23 beginnt
 %                    &%+
                       %\frac{1}{(p^- +k_1^-)(- k_1^- )} \frac{1}{p^2(p-k_2)^2} 
                     +
                      \frac{1}{(p^- +k_1^-)(-k_1^- )} \frac{1}{(p- q + k_1 )^2 (p-k_2)^2} 
\notag \\
                      &
                      %+
                      %\frac{1}{(-p^- ) (-k_1^- )} \frac{1}{p^2(p-q + k_1 + k_2)^2} 
                      +
                      \frac{1}{(-p^-)(-k_1^- )} \frac{1}{(p- q + k_1 )^2 (p-q + k_1 + k_2)^2}
%\notag \\ %%4I1 beginnt
                     %&
                     + \frac{1}{(p^- -k_1^-)(- k_1^- - k_2^- )} \frac{1}{p^2(p-k_1)^2} 
                      %+\frac{1}{(-p^- )(-k_1^- - k_2^- )} \frac{1}{p^2 (p-k_1)^2} 
\notag \\ %%4I2 beginnt
                      &%+
                      %\frac{1}{(p^- - k_1^- -k_2^- ) (-k_1^- - k_2^- )} \frac{1}{p^2(p- k_2)^2} 
                      + \frac{1}{(p^- - k_1^- - k_2^- ) (-k_1^-) } \frac{1}{p^2(p- k_2)^2} 
%\notag \\
                      %&
                      +             
                      \frac{1}{(-p^- -k_1^-) (-k_1^- -k_2^- )} \frac{1}{p^2(p- k_2)^2} 
                      %- \frac{1}{(-p^- k_1^- ) (-k_1^- )} \frac{1}{p^2(p- k_2)^2} 
\notag \\ %%4I3 beginnt                     
                      &+  
                      \frac{1}{(p^- + k_1^- + k_2^-)k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2} 
                      %+\frac{1}{(-p^- )k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2}
\bigg]
\end{align}
Next we collect terms from (3I12) and (3I23)
\begin{align}
  \label{eq:82}
E_1 &=  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{g^4{\bm{q}}^2}{p^2(p-k_1 - k_2)^2} \frac{6}{k_1^- + k_2^-} 
\bigg[ 
     \frac{2p^+}{(p-k_1)^2} - \frac{2p^+}{(p-k_2)^2}
\bigg]
\notag \\
&+
 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\frac{g^4{\bm{q}}^2}{p^2(p- q +k_1)^2} \frac{6}{k_1^- } 
\bigg[ 
     \frac{2p^+}{(p-k_2)^2} - \frac{2p^+}{(p- q + k_1 +k_2)^2}
\bigg]
\end{align}
The following terms emerge from (4I1), (4I2) and (4I3):
\begin{align}
  \label{eq:96}
F_1= \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
-16g^4 {\bm{q}}^2 
\bigg[
     \frac{1}{p^2(p-k_1)^2} 
     + 
     \frac{1}{p^2(p-k_2)^2} 
     + 
     \frac{1}{p^2(p-q + k_1 +k_2)^2}
\bigg]
 \frac{1}{(k_1^- + k_2^-)k_1^-}
\end{align}
The terms that  remain which originate from (3I12) and (3I23) are given by
\begin{align}
  \label{eq:97}
G_1 &= 8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p-k_1 - k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+ (k_1^- + k_2^-)} 
\bigg(
     \frac{p^+}{(p-k_1)^2} \frac{1}{-p^-}
     +
     \frac{p^+}{(p-k_2)^2} \frac{1}{p - k_1^- - k_2^-}
\bigg)
\notag \\
&+
8g^4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p-q +k_1 )^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+ (- k_1^- )} 
\bigg(
     \frac{p^+}{(p-k_2)^2} \frac{1}{-p^-}
     +
     \frac{p^+}{(p- q + k_1 +k_2)^2} \frac{1}{p + k_1^- }
\bigg)
\end{align}
and those from  (4I1), (4I2) and (4I3) by
\begin{align}
  \label{eq:98}
H_1 =&
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p-k_1 )^2} \frac{{\bm{k}}_1^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
\frac{1}{p^--k_1^-} + \frac{1}{p^-}
\bigg)
\notag \\
&+
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p-k_2 )^2} \frac{{\bm{k}}_2^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
\frac{1}{p^--k_1^- - k_2^-} + \frac{1}{p^- + k_1^-}
\bigg)
\notag \\
&+
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p-q + k_1 + k_2 )^2} \frac{{\bm{k}}_3^2}{p^+(-k_1^- - k_2^-) (-k_1^-)}
\bigg(
\frac{1}{p^- + k_1^- + k_2^-} + \frac{1}{p^-}
\bigg)
\end{align}


\subsubsection{$\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})$ contributions}

Using (4RRP), (4G+12), (4G+23), (GH213a), (GH213b) we find, exhausting the GH diagrams
\begin{align}
  \label{eq:99}
A_3 &= g^4 \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } (p^+)^3 p^- \big(
17 + 2 - 18 -1
\big) = 0
 \\
\label{eq:101}
A_4 &= g^4  \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 }  (p^+)^3 p^- \big(
17 + 2 - 18 -1
\big)
 =0
\end{align}
Using (4RRP), (4G+12), (4G+13),  we find, exhausting (4G+ij)
\begin{align}
  \label{eq:102}
B_2 &= g^4 \frac{(p^+)^2 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } \big(
-{\bm{p}}^2 - ({\bm{p}} - {\bm{q}})^2 - 32 {\bm{q}}^2+  8 \frac{{\bm{q}}^4}{p^+p^-}  + 18  ({\bm{p}} - {\bm{q}})^2
\big)
\notag \\
&+ 
g^4 \frac{ (p^+)^2\tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 }  \big(
-{\bm{p}}^2 - ({\bm{p}} - {\bm{q}})^2 - 32 {\bm{q}}^2+  8 \frac{{\bm{q}}^4}{p^+p^-}  + 18  ({\bm{p}} - {\bm{q}})^2
\big).
\end{align}
Using (4RPP), (3I12), (3I13) we find, exhausting (4RPP)
\begin{align}
  \label{eq:103}
C_2 &= g^46p^+  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
 \bigg[ \big(
    \frac{1}{(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
    +
    \frac{1}{p^2(p - k_2)^2 (p- k_1 - k_2)^2  }
\notag \\
&+ 
     \frac{ 1}{(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
     +
     \frac{ 1}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2  } \big) \frac{{\bm{q}}^2}{p^-}
\notag \\ %% jetzt die 3I12
&- 
      \frac{1}{p^2 (p-k_1)^2 (p - k_1 - k_2)^2 }  \frac{{\bm{q}}^2}{p^- - k_1^- - k_2^-} 
     -
      \frac{1}{p^2 (p-k_2)^2 (p - k_1 - k_2)^2 }  \frac{{\bm{q}}^2}{p^-}
\notag \\ %% jetzt die 3I13 
&-
     \frac{1}{p^2 (p-k_1)^2(p-q + k_2)^2}  \frac{{\bm{q}}^2}{p^- + k_2^-} 
    -
     \frac{1}{p^2 (p-q + k_2)^2(p-q +k_1 + k_2)^2}  \frac{{\bm{q}}^2}{p^- } 
\bigg]
\notag \\
=& %% zweites ==
 g^46p^+  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
 \bigg[ \big(
    \frac{1}{(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
    +
    %\frac{1}{p^2(p - k_2)^2 (p- k_1 - k_2)^2  }
\notag \\
&+ 
     \frac{ 1}{(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
     +
    % \frac{ 1}{p^2(p - q+ k_2)^2 (p-q + k_1 + k_2)^2  } 
\big) \frac{{\bm{q}}^2}{p^-}
\notag \\ %% jetzt die 3I12
&- 
      \frac{1}{p^2 (p-k_1)^2 (p - k_1 - k_2)^2 }  \frac{{\bm{q}}^2}{p^- - k_1^- - k_2^-} 
     -
     % \frac{1}{p^2 (p-k_2)^2 (p - k_1 - k_2)^2 }  \frac{{\bm{q}}^2}{p^-}
%\notag \\ %% jetzt die 3I13 
%&-
     \frac{1}{p^2 (p-k_1)^2(p-q + k_2)^2}  \frac{{\bm{q}}^2}{p^- + k_2^-} 
   % -
     %\frac{1}{p^2 (p-q + k_2)^2(p-q +k_1 + k_2)^2}  \frac{{\bm{q}}^2}{p^- } 
\bigg]
\end{align}
Using contributions from (3I12), (3I13), (4I1), (4I2), (4I3) we find
\begin{align}
  \label{eq:100}
D_2 &=g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})\bigg[
    \frac{1}{(p-k_2)^2(p - k_1 - k_2)^2 } \frac{1}{-p^- (k_1^- + k_2^-)} 
    + 
    \frac{1}{(p-k_2)^2p^2 } \frac{1}{-p^- (k_1^- + k_2^-)}
\notag \\
&+
    \frac{1}{(p- k_1)^2 (p - k_1 - k_2)^2} \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)}
    +
    \frac{1}{(p- k_1)^2 p^2} \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)}
\notag \\ %%3I13
&+
    \frac{1}{(p-k_1)^2(p-q + k_2)^2} \frac{1}{(p^- + k_2^-) (-k_2^-)}
    +
     \frac{1}{(p-k_1)^2p^2} \frac{1}{(p^- + k_2^-) (-k_2^-)}
\notag \\
&+
    \frac{1}{(p -q + k_2)^2 (p -q + k_1 + k_2)^2} \frac{1}{p^-k_2^-}
    +
    \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{p^-k_2^-}
\notag \\ %% 4I1 beginnt
&-
    \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- - k_1^- - k_2^-) (k_1^- + k_2^-)}  
    +
    \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- + k_2^-) (k_1^- + k_2^-)} 
\notag \\
&-
     \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- -k_1^- - k_2^-)  k_2^-}
     +
      \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- + k_2^-)  k_2^-}
\notag \\ %% 4I2 beginnt
&-
     \frac{1}{p^2(p-k_2)^2} \frac{1}{(p^- - k_2^-)(k_1^- + k_2^-)}
     +
     \frac{1}{p^2(p-k_2)^2} \frac{1}{p^- (k_1^- + k_2^-)}
\notag \\ %% 4I3 beginnt
&+
      \frac{1}{p^2(p-q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^- + k_2^-)k_2^-}
      -
      \frac{1}{p^2(p-q + k_1 + k_2)^2} \frac{1}{p^- k_2^-}
\bigg]
\notag \\
=& %% zweites ==
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})\bigg[
    \frac{1}{(p-k_2)^2(p - k_1 - k_2)^2 } \frac{1}{-p^- (k_1^- + k_2^-)} 
    %+ 
    %\frac{1}{(p-k_2)^2p^2 } \frac{1}{-p^- (k_1^- + k_2^-)}
\notag \\
&+
    \frac{1}{(p- k_1)^2 (p - k_1 - k_2)^2} \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)}
    %+
    %\frac{1}{(p- k_1)^2 p^2} \frac{1}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)}
%\notag \\ %%3I13
%&
+
    \frac{1}{(p-k_1)^2(p-q + k_2)^2} \frac{1}{(p^- + k_2^-) (-k_2^-)}
    %+
    % \frac{1}{(p-k_1)^2p^2} \frac{1}{(p^- + k_2^-) (-k_2^-)}
\notag \\
&+
    \frac{1}{(p -q + k_2)^2 (p -q + k_1 + k_2)^2} \frac{1}{p^-k_2^-}
    %+
    %\frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{p^-k_2^-}
%\notag \\ %% 4I1 beginnt
%&%-
 %   \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- - k_1^- - k_2^-) (k_1^- + k_2^-)}  
    +
    \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- + k_2^-) (k_1^- + k_2^-)} 
\notag \\
&-
     \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- -k_1^- - k_2^-)  k_2^-}
     %+
     % \frac{1}{p^2 (p-k_1)^2} \frac{1}{(p^- + k_2^-)  k_2^-}
%\notag \\ %% 4I2 beginnt
%&
-
     \frac{1}{p^2(p-k_2)^2} \frac{1}{(p^- - k_2^-)(k_1^- + k_2^-)}
     %+
     %\frac{1}{p^2(p-k_2)^2} \frac{1}{p^- (k_1^- + k_2^-)}
\notag \\ %% 4I3 beginnt
&+
      \frac{1}{p^2(p-q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^- + k_2^-)k_2^-}
      %-
      %\frac{1}{p^2(p-q + k_1 + k_2)^2} \frac{1}{p^- k_2^-}
\bigg]
\end{align}
Using contributions from (3I12), (3I13) we find
\begin{align}
  \label{eq:104}
E_2 &=
12 g^4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p - k_1 - k_2)^2} \big(
\frac{p^+}{(p-k_2)^2} - \frac{p^+}{(p - k_1)^2}
\big)
\frac{1}{k_1^- + k_2^-}
\notag \\
& +
12 g^4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})\frac{{\bm{q}}^2}{p^2 (p - q +  k_2)^2} \big(
\frac{p^+}{(p-k_1)^2} - \frac{p^+}{(p - q +k_1)^2}
\big)
\frac{1}{ k_2^-}
\end{align}
From (4I1), (4I2) and (4I3) we find
\begin{align}
  \label{eq:105}
F_2 &= -16 g^4 {\bm{q}}^2 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) \big[
\frac{1}{p^2 (p - k_1)^2} + \frac{1}{p^2 (p-k_2)^2}  + \frac{1}{p^2 (p -q + k_1 + k_2)^2}
\big] \frac{1}{(k_2^- (k_1^- + k_2^-))}
\end{align}
Using  now contributions from (3I12), (3I13) which exhaust them we find
\begin{align}
  \label{eq:106}
G_2 &=
g^4 8 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})\bigg[\frac{{\bm{q}}^2}{p^2 (p - k_1 - k_2)^2} 
\frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+(k_1^- + k_2^-)}
\bigg(
\frac{p^+}{(p - k_2)^2} \frac{1}{-p^-} + \frac{p^+}{(p - k_1)^2} \frac{1}{p^- - k_1^- - k_2^-}
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p - q  + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+(- k_2^-)}
 \bigg(
\frac{p^+}{(p - k_1)^2} \frac{1}{(p^- + k_2^-)} + \frac{p^+}{(p -q + k_1 + k_2)^2} \frac{1}{-p^-}
\bigg)\bigg]
\end{align}
Using contributions from  (4I1), (4I2) and (4I3) we find, while exhausting them
\begin{align}
  \label{eq:107}
H_2 &=8g^4\tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) \bigg[
\frac{{\bm{q}}^2}{p^2 (p- k_1)^2} \frac{{\bm{k}}_1^2}{p^+k_2^-(k_1^- + k_2^-)} 
\bigg(
     \frac{1}{p^- - k_1^- - k_2^-} + \frac{1}{p^- + k_2^-}   
\bigg)
\notag \\
&+ \frac{{\bm{q}}^2}{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{p^+ k_2^- (k_1^- + k_2^-)}
 \bigg(
      \frac{1}{p^-  - k_2^-} + \frac{1}{p^- }   
\bigg)
\notag \\
&+
 \frac{{\bm{q}}^2}{p^2 (p- q + k_1 + k_2)^2} \frac{{\bm{k}}_3^2}{p^+k_2^-(k_1^- + k_2^-)}
 \bigg(
      \frac{1}{p^-  + k_1^- + k_2^-} + \frac{1}{p^- }   
\bigg)
\bigg]
\end{align}


\subsubsection{$ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})$ contributions}
Using (4RRP), (4G+13), (4G+23), (GH132a), (GH132b) we find, exhausting the GH diagrams
\begin{align}
  \label{eq:108}
A_5 &= 
g^4\frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - k_1)^2 (p- q + k_2)^2 (p-q)^2 } \big(17 + 2 - 18 -1 \big)(p^+)^3p^- = 0
 \\
\label{eq:109}
A_6 &=
\frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - q+ k_1)^2 (p-  k_2)^2 (p-q)^2 }
 \big(17 + 2 - 18 -1 \big)(p^+)^3p^- = 0
\end{align}
Using (4RRP), (4G+13), (4G+23),  we find, exhausting (4G+ij)
\begin{align}
  \label{eq:110}
B_3 &=g^4  \frac{(p^+)^2 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - k_1)^2 (p- q + k_2)^2 (p-q)^2 }  \big(
-{\bm{p}}^2 - ({\bm{p}} - {\bm{q}})^2 - 32 {\bm{q}}^2+  8 \frac{{\bm{q}}^4}{p^+p^-}  + 18  ({\bm{p}} - {\bm{q}})^2
\big)
\notag \\
&+
g^4
\frac{(p^+)^2 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2(p - q+ k_1)^2 (p-  k_2)^2 (p-q)^2 }
\big(
-{\bm{p}}^2 - ({\bm{p}} - {\bm{q}})^2 - 32 {\bm{q}}^2+  8 \frac{{\bm{q}}^4}{p^+p^-}  + 18  ({\bm{p}} - {\bm{q}})^2
\big)
\end{align}
Using (4RPP), (3I13), (3I23) we find, exhausting (4RPP)
\begin{align}
  \label{eq:111}
C_3 &=  g^4 6p^+  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
\big( 
     \frac{1}{p^2(p - k_1)^2 (p- q + k_2)^2  } 
     + 
     \frac{1}{(p - k_1)^2 (p- q +  k_2)^2 (p-q)^2 }
\notag \\
&+
     \frac{1}{(p - q+ k_1)^2 (p- k_2)^2 (p-q)^2 }
     +
     \frac{1}{p^2(p - q+ k_1)^2 (p- k_2)^2  } 
\big)\frac{{\bm{q}}^2}{p^-}
\notag \\
&-
    \frac{1}{p^2(p - k_1)^2 (p- q + k_2)^2  } \frac{{\bm{q}}^2}{p^-}
    -
    \frac{1}{p^2 (p- q + k_2)^2 (p - q + k_1 + k_2)^2 } \frac{{\bm{q}}^2}{p^- + k_2^-}
\notag \\
&-
   \frac{1}{p^2 (p- k_2)^2 (p -q + k_1)^2} \frac{{\bm{q}}^2}{p^-}
   -
   \frac{1}{p^2 (p - q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{{\bm{q}}^2}{p^- + k_1^-}
\bigg]
\notag \\
 &= %% zweites ==
  g^4 6p^+  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
\big( 
     %\frac{1}{p^2(p - k_1)^2 (p- q + k_2)^2  } 
     %+ 
     \frac{1}{(p - k_1)^2 (p- q +  k_2)^2 (p-q)^2 }
%\notag \\
%&
+
   %  \frac{1}{(p - q+ k_1)^2 (p- k_2)^2 (p-q)^2 }
     %+
     \frac{1}{p^2(p - q+ k_1)^2 (p- k_2)^2  } 
\big)\frac{{\bm{q}}^2}{p^-}
\notag \\
&-
    %\frac{1}{p^2(p - k_1)^2 (p- q + k_2)^2  } \frac{{\bm{q}}^2}{p^-}
    %-
    \frac{1}{p^2 (p- q + k_2)^2 (p - q + k_1 + k_2)^2 } \frac{{\bm{q}}^2}{p^- + k_2^-}
%%%%%\notag \\
%&-
  % \frac{1}{p^2 (p- k_2)^2 (p -q + k_1)^2} \frac{{\bm{q}}^2}{p^-}
   -
   \frac{1}{p^2 (p - q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{{\bm{q}}^2}{p^- + k_1^-}
\bigg]
\end{align}
Using contributions from (3I13), (3I23), (4I1), (4I2), (4I3) we find
\begin{align}
  \label{eq:112}
D_3 &=
g^4 4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
     \frac{1}{(p-k_1)^2 (p- q + k_2)^2} \frac{1}{p^-k_2^-} 
     +
     \frac{1}{(p-k_1)^2 p^2} \frac{1}{p^-k_2^-} 
\notag \\
&-
     \frac{1}{ (p- q + k_2)^2 (p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-} 
     -
     \frac{1}{p^2  (p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-}  
\notag \\
&+
      \frac{1}{(p - k_2)^2 (p - q + k_1)^2} \frac{1}{p^-k_1^-} 
      +
       \frac{1}{(p - k_2)^2 p^2} \frac{1}{p^-k_1^-} 
\notag \\
&-
      \frac{1}{(p -q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
      -
      \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
\notag \\ %% 4I1 beginnt
&+
       \frac{1}{p^2(p-k_1)^2} \frac{1}{(p^- - k_1^-)  k_2^-} 
       -
       \frac{1}{p^2(p-k_1)^2} \frac{1}{p^-   k_2^-} 
\notag \\ %% 4I2 beginnt
&+
       \frac{1}{p^2(p - k_2)^2}\frac{1}{(p^- - k_2^-)k_1^-}
       -
        \frac{1}{p^2(p - k_2)^2}\frac{1}{p^-k_1^-}
\notag \\ %% 4I3 beginnt
&+
       \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-}
       -
       \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_2^-} 
\notag \\
&-
        \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_1^-}
        +
         \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
\bigg]
\notag \\
&= %% zweites ==
g^4 4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
     \frac{1}{(p-k_1)^2 (p- q + k_2)^2} \frac{1}{p^-k_2^-} 
    % +
    % \frac{1}{(p-k_1)^2 p^2} \frac{1}{p^-k_2^-} 
\notag \\
&
-
     \frac{1}{ (p- q + k_2)^2 (p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-} 
     %-
     %\frac{1}{p^2  (p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-}  
%\notag \\
%&
+
      \frac{1}{(p - k_2)^2 (p - q + k_1)^2} \frac{1}{p^-k_1^-} 
      %+
      % \frac{1}{(p - k_2)^2 p^2} \frac{1}{p^-k_1^-} 
\notag \\
&-
      \frac{1}{(p -q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
     % -
      %\frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
%\notag \\ %% 4I1 beginnt
%&
+
       \frac{1}{p^2(p-k_1)^2} \frac{1}{(p^- - k_1^-)  k_2^-} 
      % -
      % \frac{1}{p^2(p-k_1)^2} \frac{1}{p^-   k_2^-} 
\notag \\ %% 4I2 beginnt
&+
       \frac{1}{p^2(p - k_2)^2}\frac{1}{(p^- - k_2^-)k_1^-}
     %  -
     %   \frac{1}{p^2(p - k_2)^2}\frac{1}{p^-k_1^-}
%\notag \\ %% 4I3 beginnt
%&%+
  %     \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-}
       -
       \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_2^-} 
\notag \\
&
-
        \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_1^-}
   %     +
   %      \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-}
\bigg]
\end{align}
Using contributions from (3I13), (3I23) we find
\begin{align}
  \label{eq:113}
E_3 &=
12 g^4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})\frac{{\bm{q}}^2}{p^2 (p - q + k_2)^2} 
\big(
\frac{p^+}{(p - q + k_1 + k_2)^2} - \frac{p^+}{(p - k_1)^2}
\big)\frac{1}{k_2^-}
\notag \\
&+
12 g^4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})\frac{{\bm{q}}^2}{p^2 (p - q + k_1)^2} 
\big(
\frac{p^+}{(p - q + k_1 + k_2)^2} - \frac{p^+}{(p - k_2)^2}
\big)\frac{1}{k_1^-}
\end{align}
From (4I1), (4I2) and (4I3) we find
\begin{align}
  \label{eq:114}
F_3 =  16 g^4 {\bm{q}}^2 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) 
\big[
\frac{1}{p^2 (p-k_1)^2} + \frac{1}{p^2 (p - k_2)^2} + \frac{1}{p^2 (p - q + k_1 + k_2)^2}
\big]\frac{1}{k_1^-k_2^-}
\end{align}
Using  now contributions from (3I13), (3I23) which exhaust them we find
\begin{align}
  \label{eq:115}
G_3 &=
g^4 8 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
\frac{{\bm{q}}^2}{p^2 (p -q + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_1)^2} \frac{1}{p^-k_2^-} 
      -
      \frac{p^+}{(p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_2^-)k_2^-} 
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p -q + k_1)^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_2)^2} \frac{1}{p^-k_1^-} 
      -
      \frac{p^+}{(p - q + k_1 + k_2)^2} \frac{1}{(p^- + k_1^-)k_1^-} 
\bigg)
\bigg]
\end{align}
Using contributions from  (4I1), (4I2) and (4I3) we find, while exhausting them
\begin{align}
  \label{eq:116}
H_3 &=8g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) 
\bigg[
\frac{{\bm{q}}^2 }{p^2 (p- k_1)^2} \frac{{\bm{k}}_1^2}{p^+}
\frac{1}{-k_1^-k_2^-}
\bigg(
     \frac{1}{(p^- - k_1^-)} 
     +
     \frac{1}{p^-} 
\bigg)
\notag \\
&+
   \frac{{\bm{q}}^2 }{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{p^+}
\frac{1}{-k_1^-k_2^-}
\bigg(
     \frac{1}{(p^- - k_2^-)} 
     +
     \frac{1}{p^- }
\bigg)
\notag \\
&+
 \frac{{\bm{q}}^2 }{p^2 (p- q + k_1 + k_2)^2} \frac{{\bm{k}}_3^2}{p^+}
\frac{1}{-k_1^-k_2^-}  
 \bigg(
         \frac{1}{(p^- + k_1^-)} 
     +
     \frac{1}{(p^- + k_2^-) }
   \bigg)
\bigg]
\end{align}


\subsection{Cancelations using translational invariance of the loop integral}
\label{sec:canc_loop}

We consider the above expressions together with the integral over the gluon loop momentum $p$. Poles in $p^\pm$ are regularized using the Mellin transfrom of the theta-function as discussed in the case of the  gluon trajectory. Here we only keep the Regge factors like $(p^+)^\omega$ etc. while the remaining integral over $\omega$ will be inserted when needed (as it is of no relevance for the to come considerations). Further note, that we will not specify the pole structure of the induced vertices at this point, but keep in mind (and use) that the reggeized gluon as negative signature and that subtitutions like $p \to -p$ are allowed by the Regge-factors i.e. they are invariant under such a operation. to denote terms we use the same letters as in the above, but with tilde in order to denote that now the integration over $p$ has been included.
\begin{align}
  \label{eq:117}
\tilde B_1=& \int \frac{d^4 p}{(2\pi)^4} g^4\frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   (p^+)^2}{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} (-{\bm{p}}^2 - ({\bm{q }} - {\bm{p}})^2  - 32 {\bm{q}}^2 + 8 \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}
\notag \\
 &+  18 ({\bm{q }} - {\bm{p}})^2 ) \notag \\
+& \int \frac{d^4 p}{(2\pi)^4}  g^4\frac{\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) (p^+)^2}{p^2 (p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} (-{\bm{p}}^2 - ({\bm{q }} - {\bm{p}})^2    - 32 {\bm{q}}^2 
\notag \\
&+
 8 \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}  
+
 18({\bm{q }} - {\bm{p}})^2 ).
\end{align}
all terms are convergent in $p^-$ and for all terms (besides the ones with explicit poles in $p^+p^-$) the $p^-$-poles lie for arbitrary values of the other momenta on the same side of the real axis and there integral vanishes. We obtain
\begin{align}
  \label{eq:118}
\tilde B_1=&  g^4 8 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})    \int\frac{d^4 p}{(2\pi)^4} 
  \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}
\notag \\
& \bigg(
         \frac{     (p^+)^2}{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2}
         +
         \frac{   (p^+)^2}{p^2 (p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
  \bigg)
\end{align}
and similar
\begin{align}
  \label{eq:119}
\tilde B_2 =&  g^4 8 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})    \int\frac{d^4 p}{(2\pi)^4} 
  \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}
\notag \\
& \bigg(
         \frac{     (p^+)^2}{p^2 (p-k_2)^2 (p-k_1 - k_2)^2 (p-q)^2}
         +
         \frac{   (p^+)^2}{p^2 (p-q +k_2)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
  \bigg)
\end{align}
and
\begin{align}
  \label{eq:120}
\tilde B_3 =&  g^4 8 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})    \int\frac{d^4 p}{(2\pi)^4} 
  \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}
\notag \\
& \bigg(
         \frac{     (p^+)^2}{p^2 (p-k_1)^2 (p- q + k_2)^2 (p-q)^2}
         +
         \frac{   (p^+)^2}{p^2 (p-q +k_1)^2 (p- k_2)^2 (p-q)^2} 
  \bigg)
\end{align}
The next class of terms vanishes completely, but needs a shift in the momentum:
\begin{align}
  \label{eq:121}
\tilde C_1 &= g^4 6\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \int \frac{d^4 p}{(2\pi)^4}\bigg[ 
\bigg(
\frac{(p^+)^2}{(p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} 
+
\notag \\
&
+
\frac{(p^+)^2}{(p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
\bigg)
\frac{{\bm{q}}^2}{p^+p^-} (p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\
 &
-
  \frac{(p^+)^2}{p^2 (p-k_2)^2 (p-k_1 - k_2)^2 } \frac{{\bm{q}}^2}{p^+ (p^- - k_1^- - k_2^-) }  (p^+)^{\omega_1} (p^- - k_1^- -k_2^-)^{\omega_2}   \notag \\
&-
   \frac{(p^+)^2}{p^2 (p-k_2)^2 (p-q + k_1 )^2 } \frac{{\bm{q}}^2}{ p^+ (p^- + k_1^-) } (p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}
\bigg]
\notag \\
=& %%zweites ==
 g^4 6\tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \int \frac{d^4 p}{(2\pi)^4}\bigg[ 
\bigg(
\frac{(p^+)^2}{(p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2} 
+
\notag \\
&
+
\frac{(p^+)^2}{(p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
\bigg)
\frac{{\bm{q}}^2}{p^+p^-} (p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\
 &
-
  \frac{(p^+)^2}{(p - q + k_1 + k_2)^2 (p-q + k_1)^2 (p-q)^2 } \frac{{\bm{q}}^2}{p^+ p^-  }  (p^+)^{\omega_1} (p^- )^{\omega_2}   \notag \\
&-
   \frac{(p^+)^2}{(p-k_1)^2 (p-k_1 - k_2)^2 (p-q )^2 } \frac{{\bm{q}}^2}{ p^+ p^-  } (p^+)^{\omega_1}(p^- )^{\omega_2}
\bigg] = 0
\end{align}
\begin{align}
  \label{eq:122}
\tilde C_2 =&
 g^4 6  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
 \int \frac{d^4 p}{(2\pi)^4}
 \bigg[ \big(
    \frac{(p^+)^2}{(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
    \notag \\
&+ 
     \frac{ (p^+)^2}{(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
     +
    \big) \frac{{\bm{q}}^2}{p^+ p^-} (p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\ %% jetzt die 3I12
&- 
      \frac{(p^+)^2}{p^2 (p-k_1)^2 (p - k_1 - k_2)^2 }  \frac{{\bm{q}}^2}{p^+(p^- - k_1^- - k_2^-)}  (p^+)^{\omega_1}(p^- - k_1^- - k_2^-)^{\omega_2}
\notag \\    
 &-
         \frac{(p^+)^2}{p^2 (p-k_1)^2(p-q + k_2)^2}  \frac{{\bm{q}}^2}{p^+(p^- + k_2^-)} (p^+)^{\omega_1}(p^- +k_2^-)^{\omega_2}
        \bigg]
\notag \\
=& %%zweites ==
 g^4 6  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
 \int \frac{d^4 p}{(2\pi)^4}
 \bigg[ \big(
    \frac{(p^+)^2}{(p - k_2)^2 (p- k_1 - k_2)^2 (p-q)^2 } 
    \notag \\
&+ 
     \frac{ (p^+)^2}{(p - q+ k_2)^2 (p-q + k_1 + k_2)^2 (p-q)^2 } 
     +
    \big) \frac{{\bm{q}}^2}{p^+ p^-} (p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\ %% jetzt die 3I12
&- 
      \frac{(p^+)^2}{(p - q + k_1 + k_2)^2 (p-q + k_2)^2 (p - q)^2 }  \frac{{\bm{q}}^2}{p^+p^- }  (p^+)^{\omega_1}(p^- )^{\omega_2}
\notag \\    
 &-
         \frac{(p^+)^2}{(p - k_2)^2 (p-k_1 - k_2)^2(p-q )^2}  \frac{{\bm{q}}^2}{p^+p^- } (p^+)^{\omega_1}(p^- )^{\omega_2}
        \bigg] = 0
\end{align}
\begin{align}
  \label{eq:123}
\tilde C_3 =&
 g^4 6  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
\big( 
         \frac{(p^+)^2}{(p - k_1)^2 (p- q +  k_2)^2 (p-q)^2 }
\notag \\
&+
     \frac{(p^+)^2}{p^2(p - q+ k_1)^2 (p- k_2)^2  } 
\big)\frac{{\bm{q}}^2}{p^+p^-}(p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\
&-
    \frac{(p^+)^2}{p^2 (p- q + k_2)^2 (p - q + k_1 + k_2)^2 } \frac{{\bm{q}}^2}{p^+(p^- + k_2^-)}(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}
\notag \\ 
&  -
   \frac{(p^+)^2}{p^2 (p - q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{{\bm{q}}^2}{p^+(p^- + k_1^-)}(p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}
\bigg]
\notag \\
=& %% zweites ==
 g^4 6  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\bigg[
\big( 
         \frac{(p^+)^2}{(p - k_1)^2 (p- q +  k_2)^2 (p-q)^2 }
\notag \\
&+
     \frac{(p^+)^2}{p^2(p - q+ k_1)^2 (p- k_2)^2  } 
\big)\frac{{\bm{q}}^2}{p^+p^-}(p^+)^{\omega_1}(p^-)^{\omega_2}
\notag \\
&
-
    \frac{(p^+)^2}{(p - q + k_2)^2 p^2 (p -  k_1 )^2 } \frac{{\bm{q}}^2}{p^+p^- }(p^+)^{\omega_1}(p^- )^{\omega_2}
\notag \\ 
&  -
   \frac{(p^+)^2}{p^2 (p - q + k_1)^2 (p - k_2)^2} \frac{{\bm{q}}^2}{p^+p^- }(p^+)^{\omega_1}(p^- )^{\omega_2}
\bigg] = 0
\end{align}
The same is true for the $D_i$-terms (note that the $p^+$ regulator is introduced as every propagator-like denominator should come with a $p^+$ in the numerator - alternatively: change to $\mu_{k_i} = p^+k_i^-$ and a $p^+$-pole would arise by the Jacobian)
\begin{align}
  \label{eq:124}
\tilde D_1 =&
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \int \frac{d^4 p}{(2\pi)^4} 
\bigg[ %1
     -\frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_1)^2} 
\notag \\
     &
     +%2
     \frac{(p^+)^{\omega_1}(p^- - k_1^- -k_2^- )^{\omega_2}}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_2)^2}
  -%3
      \frac{(p^+)^{\omega_1}(p^- - k_1^- )^{\omega_2}}{(p^- -k_1^-)( k_1^- + k_2^- )} \frac{1}{p^2(p-k_1)^2} 
   \notag \\
& + %6            
      \frac{(p^+)^{\omega_1}(p^- + k_1^- )^{\omega_2}}{(p^- +k_1^-) (k_1^- +k_2^- )} \frac{1}{p^2(p- k_2)^2} 
 \notag \\
      &
      +%4
      \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-k_1^- } \frac{1}{(p- q + k_1 )^2 (p-q + k_1 + k_2)^2}
   % \notag \\ %%4I2 beginnt
%      &
-%5
      \frac{(p^+)^{\omega_1}(p^- - k_1^- - k_2^- )^{\omega_2}}{(p^- - k_1^- - k_2^- ) k_1^- } \frac{1}{p^2(p- k_2)^2}   
\notag \\ %%4I3 beginnt                     
      &+  
      \frac{(p^+)^{\omega_1}(p^- + k_1^- + k_2^- )^{\omega_2}}{(p^- + k_1^- + k_2^-)k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2} 
 -
     \frac{(p^+)^{\omega_1}(p^- + k_1^- )^{\omega_2}}{(p^- +k_1^-)k_1^- } \frac{1}{(p- q + k_1 )^2 (p-k_2)^2} 
\bigg]
\notag \\
=& %% zweites ==
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  \int \frac{d^4 p}{(2\pi)^4} 
\bigg[ %1
     -\frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-(k_1^- + k_2^-)} \frac{1}{(p- k_1 -k_2)^2 (p-k_1)^2} 
\notag \\
     &
     +%2
     \frac{(p^+)^{\omega_1}(p^- - k_1^- )^{\omega_2}}{(p^- - k_1^- )(k_1^- + k_2^-)} \frac{1}{(p- k_1 )^2 p^2}
  -%3
      \frac{(p^+)^{\omega_1}(p^- - k_1^- )^{\omega_2}}{(p^- -k_1^-)( k_1^- + k_2^- )} \frac{1}{p^2(p-k_1)^2} 
   \notag \\
& + %4            
      \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-  (k_1^- +k_2^- )} \frac{1}{(p-k_1)^2(p -k_1 - k_2)^2} 
 \notag \\
      &
      +%5
      \frac{(p^+)^{\omega_1}(p^-  )^{\omega_2}}{p^-k_1^- } \frac{1}{(p- q + k_1 )^2 (p-q + k_1 + k_2)^2}
   % \notag \\ %%4I2 beginnt
%      &
-%6
      \frac{(p^+)^{\omega_1}(p^-  )^{\omega_2}}{p^-  k_1^- } \frac{1}{(p - q + k_1 + k_2)^2(p- q +  k_1)^2}   
\notag \\ %%4I3 beginnt                     
      &+%7  
      \frac{(p^+)^{\omega_1}(p^- + k_1^- + k_2^- )^{\omega_2}}{(p^- + k_1^- + k_2^-)k_1^- } \frac{1}{p^2 (p-q + k_1 + k_2)^2} 
\notag \\
& 
-%8
     \frac{(p^+)^{\omega_1}(p^- + k_1^- +k_2^-)^{\omega_2}}{(p^- +k_1^- + k_2^-)k_1^- } \frac{1}{(p- q + k_1 +k_2)^2 p^2} 
\bigg] = 0
\end{align}
\begin{align}
  \label{eq:125}
\tilde D_2 =&
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4}
   \bigg[
    %1
    -\frac{1}{(p-k_2)^2(p - k_1 - k_2)^2 } \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^- (k_1^- + k_2^-)} 
    \notag \\
    &+%2
    \frac{1}{(p- k_1)^2 (p - k_1 - k_2)^2} \frac{(p^+)^{\omega_1}(p^- - k_1^- - k_2^-)^{\omega_2}}{(p^- - k_1^- - k_2^-)(k_1^- + k_2^-)}
    +%5
    \frac{1}{p^2 (p-k_1)^2} \frac{(p^+)^{\omega_1}(p^- +k_2^-)^{\omega_2}}{(p^- + k_2^-) (k_1^- + k_2^-)} 
    \notag \\
    &
-%7
     \frac{1}{p^2(p-k_2)^2} \frac{(p^+)^{\omega_1}(p^- - k_2^-)^{\omega_2}}{(p^- - k_2^-)(k_1^- + k_2^-)}
    -%3
    \frac{1}{(p-k_1)^2(p-q + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-) k_2^-}   
    \notag \\
    &-%6
     \frac{1}{p^2 (p-k_1)^2} \frac{(p^+)^{\omega_1}(p^- - k_1^- - k_2^-)^{\omega_2}}{(p^- -k_1^- - k_2^-)  k_2^-}
+%4
    \frac{1}{(p -q + k_2)^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^-k_2^-}    
    \notag \\ %% 4I3 beginnt
    &+%8
    \frac{1}{p^2(p-q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_1^- + k_2^-)^{\omega_2}}{(p^- + k_1^- + k_2^-)k_2^-}
    \bigg]
\notag \\
=& %%zweites ==
g^4 {\bm{q}}^2 4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4}
   \bigg[
    %1
    -\frac{1}{(p-k_2)^2(p - k_1 - k_2)^2 } \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^- (k_1^- + k_2^-)} 
    \notag \\
    &+%2
    \frac{1}{p^2 (p  - k_2)^2} \frac{(p^+)^{\omega_1}(p^-  - k_2^-)^{\omega_2}}{(p^-  - k_2^-)(k_1^- + k_2^-)}
    +%5
    \frac{1}{(p-k_2)^2 (p-k_1-k_2)^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-  (k_1^- + k_2^-)} 
    \notag \\
    &
-%7
     \frac{1}{p^2(p-k_2)^2} \frac{(p^+)^{\omega_1}(p^- - k_2^-)^{\omega_2}}{(p^- - k_2^-)(k_1^- + k_2^-)}
    -%3
    \frac{1}{(p-k_1)^2(p-q + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-) k_2^-}   
    \notag \\
    &-%6
     \frac{1}{(p-q + k_1 + k_2)^2 (p-q + k_2)^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-   k_2^-}
+%4
    \frac{1}{(p -q + k_2)^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^-k_2^-}    
    \notag \\ %% 4I3 beginnt
    &+%8
    \frac{1}{(p - k_1)^2(p-q  + k_2)^2} \frac{(p^+)^{\omega_1}(p^-  + k_2^-)^{\omega_2}}{(p^-  + k_2^-)k_2^-}
    \bigg] =0
\end{align}
\begin{align}
  \label{eq:126}
\tilde D_3 =&
g^4 4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4}
\bigg[%1
     \frac{1}{(p-k_1)^2 (p- q + k_2)^2} \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^-k_2^-} 
     \notag \\
     &
     -%2
     \frac{1}{ (p- q + k_2)^2 (p - q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)k_2^-} 
     +%5
     \frac{1}{p^2(p-k_1)^2} \frac{(p^+)^{\omega_1}(p^- - k_1^-)^{\omega_2}}{(p^- - k_1^-)  k_2^-}     
     \notag \\
     &-%7
     \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}}{(p^- + k_1^-)k_2^-} 
     +%3
     \frac{1}{(p - k_2)^2 (p - q + k_1)^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-k_1^-} 
     \notag \\ %% 4I2 beginnt
     &+%6
     \frac{1}{p^2(p - k_2)^2}\frac{(p^+)^{\omega_1}(p^- - k_2^-)^{\omega_2}}{(p^- - k_2^-)k_1^-}
     -%4
     \frac{1}{(p -q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}}{(p^- + k_1^-)k_1^-}     \notag \\
     &
     -%8
     \frac{1}{p^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)k_1^-}
   \bigg]
\notag \\
=& %%zweites ==
g^4 4 {\bm{q}}^2 4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4}
\bigg[%1
     \frac{1}{(p-k_1)^2 (p- q + k_2)^2} \frac{(p^+)^{\omega_1}(p^-)^{\omega_2}}{p^-k_2^-} 
     \notag \\
     &
     -%2
     \frac{1}{ (p- q + k_2)^2 (p - q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)k_2^-} 
\notag \\     
&+%5
     \frac{1}{(p - q + k_1 + k_2)^2(p-q + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)  k_2^-}     
     \notag \\
     &-%7
     \frac{1}{(p-k_1)^2 (p -q  + k_2)^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^- k_2^-} 
     +%3
     \frac{1}{(p - k_2)^2 (p - q + k_1)^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^-k_1^-} 
     \notag \\ %% 4I2 beginnt
     &+%6
     \frac{1}{(p - q + k_1 + k_2)^2(p -q +  k_1)^2}\frac{(p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}}{(p^- + k_1^-)k_1^-}
\notag \\  
  & -%4
     \frac{1}{(p -q + k_1)^2 (p -q + k_1 + k_2)^2} \frac{(p^+)^{\omega_1}(p^- + k_1^-)^{\omega_2}}{(p^- + k_1^-)k_1^-}     \notag \\
     &
     -%8
     \frac{1}{(p-k_2)^2 (p -q + k_1 )^2} \frac{(p^+)^{\omega_1}(p^- )^{\omega_2}}{p^- k_1^-}
   \bigg] = 0
\end{align}
\begin{align}
  \label{eq:127}
\tilde E_1 &=  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}
\frac{g^4{\bm{q}}^2}{p^2(p-k_1 - k_2)^2} \frac{6}{k_1^- + k_2^-} 
\bigg[ 
     \frac{2p^+}{(p-k_1)^2} - \frac{2p^+}{(p-k_2)^2}
\bigg] (p^+)^{\omega_1}
\notag \\
&+
 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})\int \frac{d^4 p}{(2\pi)^4}
\frac{g^4{\bm{q}}^2}{p^2(p- q +k_1)^2} \frac{6}{k_1^- } 
\bigg[ 
     \frac{2p^+}{(p-k_2)^2} - \frac{2p^+}{(p- q + k_1 +k_2)^2}
\bigg](p^+)^{\omega_1} = 0
\end{align}
as all $p^-$ poles lie on the same side of the real axis. Similar for
\begin{align}
  \label{eq:128}
\tilde E_2 &=
12 g^4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) 
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
 \frac{{\bm{q}}^2}{p^2 (p - k_1 - k_2)^2} \big(
\frac{p^+}{(p-k_2)^2} - \frac{p^+}{(p - k_1)^2}
\big)
\frac{1}{k_1^- + k_2^-}
\notag \\
& +
12 g^4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p - q +  k_2)^2} \big(
\frac{p^+}{(p-k_1)^2} - \frac{p^+}{(p - q +k_1)^2}
\big)
\frac{1}{ k_2^-} =0
\end{align}
and
\begin{align}
  \label{eq:129}
\tilde E_3 &=
12 g^4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p - q + k_2)^2} 
\big(
\frac{p^+}{(p - q + k_1 + k_2)^2} - \frac{p^+}{(p - k_1)^2}
\big)\frac{1}{k_2^-}
\notag \\
&+
12 g^4 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p - q + k_1)^2} 
\big(
\frac{p^+}{(p - q + k_1 + k_2)^2} - \frac{p^+}{(p - k_2)^2}
\big)\frac{1}{k_1^-} =0
\end{align}
They same applies to the following class of terms
\begin{align}
  \label{eq:130}
\tilde F_1=& -\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
16 g^4 {\bm{q}}^2 
\bigg[
     \frac{1}{p^2(p-k_1)^2} 
     + 
     \frac{1}{p^2(p-k_2)^2} 
\notag \\     
&+ 
     \frac{1}{p^2(p-q + k_1 +k_2)^2}
\bigg]
 \frac{1}{(k_1^- + k_2^-)k_1^-} =0
\end{align}
\begin{align}
  \label{eq:131}
\tilde F_2 =& -16 g^4 {\bm{q}}^2 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
 \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
 \big[
\frac{1}{p^2 (p - k_1)^2} + \frac{1}{p^2 (p-k_2)^2} 
\notag \\
& + \frac{1}{p^2 (p -q + k_1 + k_2)^2}
\big] \frac{1}{(k_2^- (k_1^- + k_2^-))} =0
\end{align}
\begin{align}
  \label{eq:132}
\tilde F_3 =&  16 g^4 {\bm{q}}^2 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) 
 \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\big[
\frac{1}{p^2 (p-k_1)^2} + \frac{1}{p^2 (p - k_2)^2} 
\notag \\ &
+ \frac{1}{p^2 (p - q + k_1 + k_2)^2}
\big]\frac{1}{k_1^-k_2^-} =0
\end{align}
The following terms however are non-vanishing
\begin{align}
  \label{eq:133}
\tilde G_1 &= 
-8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p-k_1 - k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+ (k_1^- + k_2^-)} 
\notag \\
&\bigg(
     \frac{p^+}{(p-k_1)^2} \frac{(p^-)^{\omega_2}}{p^-}
     -
     \frac{p^+}{(p-k_2)^2} \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- - k_2^-}
\bigg)
\notag \\
&-
8g^4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p-q +k_1 )^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+ (- k_1^- )} 
\notag \\
&\bigg(
     \frac{p^+}{(p-k_2)^2} \frac{(p^-)^{\omega_2}}{p^-}
     -
     \frac{p^+}{(p- q + k_1 +k_2)^2} \frac{(p^- +k_1^-)^{\omega_2}}{p^- + k_1^- }
\bigg)
\notag \\
&= %%zweites ==
-8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p-k_1 - k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+ (k_1^- + k_2^-)} 
\notag \\
&\bigg(
     \frac{p^+}{(p-k_1)^2} \frac{(p^-)^{\omega_2}}{p^-}
     +
     \frac{p^+}{(p-k_1)^2} \frac{(p^- )^{\omega_2}}{p^- }
\bigg)
\notag \\
&-
8g^4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\frac{{\bm{q}}^2}{p^2 (p-q +k_1 )^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+ (- k_1^- )} 
\notag \\
&\bigg(
     \frac{p^+}{(p-k_2)^2} \frac{(p^-)^{\omega_2}}{p^-}
     +
     \frac{p^+}{(p- k_2)^2} \frac{(p^- )^{\omega_2}}{p^- }
\bigg)
\notag \\
&= %%drittes ==
-16g^4 {\bm{q}}^2 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   
\int \frac{d^4 p}{(2\pi)^4}
\frac{(p^+)^2}{p^2(p - k_1)^2 (p-k_1 - k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+ (k_1^- + k_2^-)} 
     \frac{ (p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-}
\notag \\
&-
16g^4 {\bm{q}}^2 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4} 
\frac{(p^+)^2}{p^2(p - k_2)^2 (p-q +k_1 )^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+ (- k_1^- )} 
     \frac{ (p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-}
\end{align}
\begin{align}
  \label{eq:134}
\tilde G_2 =&
g^4 8 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\bigg[\frac{{\bm{q}}^2}{p^2 (p - k_1 - k_2)^2} 
\frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+(k_1^- + k_2^-)}
\bigg(
\frac{p^+}{(p - k_2)^2} \frac{(p^-)^{\omega_2}}{-p^-} 
\notag \\
&+ \frac{p^+}{(p - k_1)^2} \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- - k_2^-}
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p - q  + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+(- k_2^-)}
 \bigg(
\frac{p^+}{(p - k_1)^2} \frac{(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)} + \frac{p^+}{(p -q + k_1 + k_2)^2} \frac{(p^-)^{\omega_2}}{-p^-}
\bigg)\bigg]
\notag \\
=& %%zweites ==
-g^4 8 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\bigg[\frac{{\bm{q}}^2}{p^2 (p - k_1 - k_2)^2} 
\frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+(k_1^- + k_2^-)}
\bigg(
\frac{p^+}{(p - k_2)^2} \frac{(p^-)^{\omega_2}}{p^-} 
\notag \\
&+ \frac{p^+}{(p - k_2)^2} \frac{(p^- )^{\omega_2}}{p^- }
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p - q  + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+(- k_2^-)}
 \bigg(
\frac{p^+}{(p -q +  k_1 + k_2)^2} \frac{(p^- )^{\omega_2}}{p^- } + \frac{p^+}{(p -q + k_1 + k_2)^2} \frac{(p^-)^{\omega_2}}{p^-}
\bigg)\bigg]
\notag \\
=& % drittes ==
-g^4{\bm{q}}^2 16 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4} 
\bigg[\frac{(p^+)^2}{p^2 (p - k_2)^2 (p - k_1 - k_2)^2} 
\frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+(k_1^- + k_2^-)}
\frac{ (p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-} 
\notag \\
&+
\frac{(p^+)^2}{p^2 (p - q  + k_2)^2 (p - q + k_1 + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+(- k_2^-)}
\frac{(p^+)^{\omega_1}}{p^+} \frac{(p^- )^{\omega_2}}{p^- } 
\bigg]
\end{align}
\begin{align}
  \label{eq:135}
\tilde G_3 =&
g^4 8 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\bigg[
\frac{{\bm{q}}^2}{p^2 (p -q + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_1)^2} \frac{(p^-)^{\omega_2}}{p^-k_2^-} 
\notag \\     
& -
      \frac{p^+}{(p - q + k_1 + k_2)^2} \frac{(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-)k_2^-} 
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p -q + k_1)^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_2)^2} \frac{(p^- )^{\omega_2}}{p^-k_1^-} 
      -
      \frac{p^+}{(p - q + k_1 + k_2)^2} \frac{(p^- +k_1^-)^{\omega_2}}{(p^- + k_1^-)k_1^-} 
\bigg)
\bigg]
\notag \\
=& %% zweites ==
g^4 8 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\bigg[
\frac{{\bm{q}}^2}{p^2 (p -q + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_1)^2} \frac{(p^-)^{\omega_2}}{(-p^-)(-k_2^-)} 
\notag \\     
& +
      \frac{p^+}{(p - k_1 )^2} \frac{(p^- )^{\omega_2}}{(-p^- -)(-k_2^-)} 
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p -q + k_1)^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+}
\bigg(
      \frac{p^+}{(p - k_2)^2} \frac{(p^- )^{\omega_2}}{(-p^-)(-k_1^-)} 
      +
      \frac{p^+}{(p -  k_2)^2} \frac{(p^- )^{\omega_2}}{(-p^- )(-k_1^-)} 
\bigg)
\bigg]
\notag \\
&= %% drittes ==
-g^4 16 {\bm{q}}^2 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4} 
\bigg[
     \frac{(p^+)^2}{p^2 (p - k_1)^2(p -q + k_2)^2} \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+  )(-k_2^-)}
      \frac{(p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-} 
      \notag \\     
      &+
      \frac{(p^+)^2}{p^2 (p - k_2)^2(p -q + k_1)^2} \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+(-k_1^-)}
      \frac{(p^+)^{\omega_1}}{p^+} \frac{(p^- )^{\omega_2}}{p^-} 
\bigg]
\end{align}
\begin{align}
  \label{eq:136}
\tilde H_1 =&
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\bigg[
\frac{{\bm{q}}^2}{p^2 (p-k_1 )^2} \frac{{\bm{k}}_1^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
      \frac{(p^- - k_1^-)^{\omega_2}}{p^--k_1^-} 
      +
      \frac{(p^-)^{\omega_2}}{p^-}
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p-k_2 )^2} \frac{{\bm{k}}_2^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
      \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^--k_1^- - k_2^-} 
      +
      \frac{(p^- + k_1^-)^{\omega_2}}{p^- + k_1^-}
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p-q + k_1 + k_2 )^2} \frac{{\bm{k}}_3^2}{p^+(-k_1^- - k_2^-) (-k_1^-)}
\bigg(
      \frac{(p^- + k_1^- + k_2^-)^{\omega_2}}{p^- + k_1^- + k_2^-} 
      +
      \frac{(p^-)^{\omega_2}}{p^-}
\bigg)
\bigg]
\notag \\
=& %% zweites ==
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\bigg[
\frac{{\bm{q}}^2}{p^2 (p-k_1 )^2} \frac{{\bm{k}}_1^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
      \frac{(p^- )^{\omega_2}}{p^-} 
      +
      \frac{(p^-)^{\omega_2}}{p^-}
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{(p-k_1)^2 (p-k_1 - k_2 )^2} \frac{{\bm{k}}_2^2}{p^+(k_1^- + k_2^-) k_1^-}
\bigg(
      \frac{(p^- )^{\omega_2}}{p^-} 
      +
      \frac{(p^- )^{\omega_2}}{p^- }
\bigg)
\notag \\
&+
\frac{{\bm{q}}^2}{p^2 (p-q + k_1 + k_2 )^2} \frac{{\bm{k}}_3^2}{p^+(-k_1^- - k_2^-) (-k_1^-)}
\bigg(
      \frac{(p^- )^{\omega_2}}{p^- } 
      +
      \frac{(p^-)^{\omega_2}}{p^-}
\bigg)
\bigg]
\notag \\
=& %% drittes ==
16g^4  {\bm{q}}^2\tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) \int \frac{d^4 p}{(2\pi)^4} 
\bigg[
\frac{(p^+)^2}{p^2 (p-k_1 )^2} \frac{{\bm{k}}_1^2}{p^+(k_1^- + k_2^-) p^+k_1^-}
      \frac{(p^- )^{\omega_2}}{p^-}   \frac{(p^+ )^{\omega_1}}{p^+} 
\notag \\
&+
\frac{(p^+)^2}{(p-k_1)^2 (p-k_1 - k_2 )^2} \frac{{\bm{k}}_2^2}{p^+(k_1^- + k_2^-) p^+k_1^-}
      \frac{(p^- )^{\omega_2}}{p^-}  \frac{(p^+ )^{\omega_1}}{p^+}
\notag \\
&+
\frac{(p^+)^2}{p^2 (p-q + k_1 + k_2 )^2} \frac{{\bm{k}}_3^2}{p^+(-k_1^- - k_2^-) p^+(-k_1^-)}
      \frac{(p^-)^{\omega_2}}{p^-} \frac{(p^+)^{\omega_1}}{p^+}
\bigg]
\end{align}
\begin{align}
  \label{eq:137}
  \tilde H_2 &=8g^4 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}  \bigg[
\frac{{\bm{q}}^2}{p^2 (p- k_1)^2} \frac{{\bm{k}}_1^2}{p^+k_2^-(k_1^- + k_2^-)} 
\bigg(
      \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- - k_2^-} 
      \notag \\
      &+
      \frac{(p^- + k_2^-)^{\omega_2}}{p^- + k_2^-}   
\bigg)
%\notag \\
%&
+ \frac{{\bm{q}}^2}{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{p^+k_2^-(k_1^- + k_2^-)}
 \bigg(
      \frac{(p^- - k_2^-)^{\omega_2}}{p^-  - k_2^-} + \frac{(p^-)^{\omega_2}}{p^- }   
\bigg)
\notag \\
&+
 \frac{{\bm{q}}^2}{p^2 (p- q + k_1 + k_2)^2} \frac{{\bm{k}}_3^2}{p^+k_2^-(k_1^- + k_2^-)}
 \bigg(
      \frac{(p^- + k_1^- + k_2^-)^{\omega_2}}{p^-  + k_1^- + k_2^-} + \frac{(p^-)^{\omega_2}}{p^- }   
\bigg)
\bigg]
\notag \\
=& %% zweites ==
16 g^4 {\bm{q}}^2 \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) 
\int \frac{d^4 p}{(2\pi)^4} 
\bigg[
     \frac{(p^+)^2}{(p - k_1 - k_2)^2 (p- k_2)^2} \frac{{\bm{k}}_1^2}{p^+k_2^-p^+ (k_1^- + k_2^-)} 
      \frac{(p^- )^{\omega_2}}{p^- }  \frac{(p^+ )^{\omega_1}}{p^+ } 
\notag \\
&+
 \frac{(p^-)^{\omega_2}}{p^- }    \frac{(p^+)^{\omega_1}}{p^+ }   
\bigg(
       \frac{(p^+)^2}{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{p^+k_2^-p^+(k_1^- + k_2^-)}
%\notag \\
%&
       +
       \frac{(p^+)^2}{p^2 (p- q + k_1 + k_2)^2} \frac{{\bm{k}}_3^2}{p^+k_2^-p^+(k_1^- + k_2^-)}
\bigg)
\bigg]
\end{align}
and finally
\begin{align}
  \label{eq:138}
\tilde H_3 &=
8g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\bigg[
\frac{{\bm{q}}^2 }{p^2 (p- k_1)^2} \frac{{\bm{k}}_1^2}{p^+}
\frac{1}{-k_1^-k_2^-}
\bigg(
     \frac{(p^- - k_1^-)^{\omega_2}}{(p^- - k_1^-)} 
     +
     \frac{(p^-)^{\omega_2}}{p^-} 
\bigg)
\notag \\
&+
   \frac{{\bm{q}}^2 }{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{p^+}
\frac{1}{-k_1^-k_2^-}
\bigg(
     \frac{(p^- - k_2^-)^{\omega_2}}{(p^- - k_2^-)} 
     +
     \frac{(p^-)^{\omega_2}}{p^- }
\bigg)
\notag \\
&+
 \frac{{\bm{q}}^2 }{p^2 (p- q + k_1 + k_2)^2} \frac{{\bm{k}}_3^2}{p^+}
\frac{1}{-k_1^-k_2^-}  
 \bigg(
         \frac{(p^- + k_1^-)^{\omega_2}}{(p^- + k_1^-)} 
     +
     \frac{(p^- + k_2^-)^{\omega_2}}{(p^- + k_2^-) }
   \bigg)
\bigg]
\notag \\
=& %% zweites ==
16{\bm{q}}^2 g^4\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) \int \frac{d^4 p}{(2\pi)^4} 
\bigg[
     \frac{(p^-)^{\omega_2}}{p^-} 
     \frac{(p^+)^{\omega_1}}{p^+} 
     \bigg(
           \frac{(p^+)^2 }{p^2 (p- k_1)^2} \frac{{\bm{k}}_1^2}{-p^+ k_1^-p^+k_2^-}
           +
           \frac{(p^+)^2 }{p^2 (p- k_2)^2} \frac{{\bm{k}}_2^2}{-p^+k_1^-p^+k_2^-}
      \bigg)
      \notag \\
      &+
      \frac{(p^+)^2 }{(p-k_1)^2 (p- q + k_2)^2} \frac{{\bm{k}}_3^2}{-p^+k_1^-p^+k_2^-}  
         \frac{(p^- )^{\omega_2}}{p^-}  \frac{(p^+ )^{\omega_1}}{p^+} 
\bigg]
\end{align}


\subsubsection{List of non-zero terms}

\begin{align}
  \label{eq:139}
\tilde B =& \tilde B_1 + \tilde B_2 + \tilde B_3 =
 g^4 8   \int\frac{d^4 p}{(2\pi)^4} 
  \frac{{\bm{q}}^4}{p^+p^-}(p^+)^{\omega_1} (p^-)^{\omega_2}  (p^+)^2
\notag \\
& \bigg(
       \frac{  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})    }{p^2 (p-k_1)^2 (p-k_1 - k_2)^2 (p-q)^2}
       +
       \frac{   \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})  }{p^2 (p-q +k_1)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
       \notag \\
       &+ 
       \frac{  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})    }{p^2 (p-k_2)^2 (p-k_1 - k_2)^2 (p-q)^2}
       +
       \frac{   \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})  }{p^2 (p-q +k_2)^2 (p-q +k_1 + k_2)^2 (p-q)^2} 
       \notag \\
       &+
       \frac{  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})   }{p^2 (p-k_1)^2 (p- q + k_2)^2 (p-q)^2}
       +
       \frac{  \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) }{p^2 (p-q +k_1)^2 (p- k_2)^2 (p-q)^2} 
\bigg)
\end{align}
\begin{align}
  \label{eq:140}
\tilde G =& \tilde G_1 + \tilde G_2 + \tilde G_3 = -16g^4 {\bm{q}}^2 \int \frac{d^4 p}{(2\pi)^4} (p^+)^2
\notag \\
&
\bigg[
      \frac{({\bm{k}}_1 + {\bm{k}}_2)^2}{p^+ (k_1^- + k_2^-)} 
      \frac{ (p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-}
      \bigg(
            \frac{  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{p^2(p - k_1)^2 (p-k_1 - k_2)^2}
            +
            \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2 (p - k_2)^2 (p - k_1 - k_2)^2} 
      \bigg)
      \notag \\
      &+
       \frac{({\bm{k}}_2 + {\bm{k}}_3)^2}{p^+ (- k_1^- )} 
      \frac{ (p^+)^{\omega_1}}{p^+} \frac{(p^-)^{\omega_2}}{p^-}
      \bigg(
            \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{p^2(p - k_2)^2 (p-q +k_1 )^2} 
            +
            \frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2 (p - k_2)^2(p -q + k_1)^2}
     \bigg)
     \notag \\
      &+
      \frac{({\bm{k}}_1 + {\bm{k}}_3)^2}{p^+(- k_2^-)}
      \frac{(p^+)^{\omega_1}}{p^+} \frac{(p^- )^{\omega_2}}{p^- } 
      \bigg(
            \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3})}{p^2 (p - q  + k_2)^2 (p - q + k_1 + k_2)^2}
            +
            \frac{ \tr(T^{a}T^{b_1}T^{b_3}T^{b_2})}{p^2 (p - k_1)^2(p -q + k_2)^2} 
      \bigg)
\bigg]
\end{align}
\begin{align}
\label{eq:142}
\tilde H =& \tilde H_1 + \tilde H_2 + \tilde H_3 = \tilde H_a + \tilde H_b  
\end{align}
where
\begin{align}
  \label{eq:141}
 \tilde H_a =& 16g^4 {\bm{q}}^2  \int \frac{d^4 p}{(2\pi)^4} 
%\notag \\
%&
\bigg[ 
 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) 
     \frac{(p^+)^2}{(p-k_1)^2 (p -k_1 - k_2 )^2}
     \frac{{\bm{k}}_2^2}{p^+(k_1^- + k_2^-) p^+k_1^-}
     \frac{(p^- )^{\omega_2}}{p^-}  \frac{(p^+ )^{\omega_1}}{p^+}
\notag \\
&+
  \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) 
        \frac{(p^+)^2}{(p - k_1 - k_2)^2 (p- k_2)^2} 
        \frac{{\bm{k}}_1^2}{p^+k_2^-p^+ (k_1^- + k_2^-)} 
        \frac{(p^- )^{\omega_2}}{p^- }  \frac{(p^+ )^{\omega_1}}{p^+ } 
\notag \\
&+
 \tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) 
       \frac{(p^+)^2 }{(p-k_1)^2 (p- q + k_2)^2}
       \frac{{\bm{k}}_3^2}{p^+k_1^-(-p^+k_2^-)}  
       \frac{(p^- )^{\omega_2}}{p^-}  \frac{(p^+ )^{\omega_1}}{p^+} 
\end{align}
\begin{align}
  \label{eq:143}
\tilde H_b =& 16g^4 {\bm{q}}^2  \int \frac{d^4 p}{(2\pi)^4}  \frac{(p^- )^{\omega_2}}{p^-}   \frac{(p^+ )^{\omega_1}}{p^+} \frac{(p^+)^2}{p^2}
\notag \\
&
\bigg[
     \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3}) }{ (p-k_1 )^2} 
     \frac{{\bm{k}}_1^2}{p^+(k_1^- + k_2^-) p^+k_1^-} 
     +
     \frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2}) }{ (p- k_1)^2} 
     \frac{{\bm{k}}_1^2}{-p^+ k_1^-p^+k_2^-}
     \notag \\
     &+
     \frac{ \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})}{ (p-q + k_1 + k_2 )^2}
     \frac{{\bm{k}}_3^2}{p^+(-k_1^- - k_2^-) p^+(-k_1^-)}
     +
     \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) }{ (p- q + k_1 + k_2)^2} 
     \frac{{\bm{k}}_3^2}{p^+k_2^-p^+(k_1^- + k_2^-)}
     \notag \\
     &+
     \frac{ \tr(T^{a}T^{b_2}T^{b_1}T^{b_3}) }{ (p- k_2)^2} 
     \frac{{\bm{k}}_2^2}{p^+k_2^-p^+(k_1^- + k_2^-)}
     +
     \frac{\tr(T^{a}T^{b_1}T^{b_3}T^{b_2})  }{ (p- k_2)^2}
     \frac{{\bm{k}}_2^2}{-p^+k_1^-p^+k_2^-}
 \bigg]
\end{align}
Note that these terms resemble the 2-to-3 reggeized gluons transition kernel. 

\subsubsection{Complication due to the pole structure of the induced vertex}

For the induced vertices the following pole structure should be used. We have
\begin{align}
  \label{eq:145}
\Delta_-^{c_1c_3b_3a}&(-p^-, p^- - k^-, k^-) =ig^2 {\bm{q}}^2 \big[
\frac{f^{b_3 c_1e} f^{c_3e a}}{k^- (p^- - k^-)} + \frac{f^{b_3c_3e} f^{c_1ea}}{k^- (-p^-) }
\big] (n^-)^\mu (n^-)^\nu 2
\end{align}
with the poles given by
\begin{align}
  \label{eq:144}
  \frac{f^{b_3 c_1e} f^{c_3e a}}{k^- (p^- - k^-)} &+ \frac{f^{b_3c_3e} f^{c_1ea}}{k^- (-p^-) }  =
\notag \\
=-\frac{f^{b_3 c_1e} f^{c_3e a}}{3!} 
&\bigg(
      \frac{2}{(-k^- +i\epsilon)(p^- - k^- + i\epsilon)} 
      +
      \frac{2}{(k^- +i\epsilon)(-p^- + k^- + i\epsilon)} 
      \notag \\
     &
      -
      \frac{1}{(-k^- + i\epsilon)(-p^- +i\epsilon)}
      -
      \frac{1}{(k^- + i\epsilon)(p^- +i\epsilon)}
      \notag \\
      &
      -
      \frac{1}{(p^- +i\epsilon)(p^- - k^- +i\epsilon)}
      -
     \frac{1}{(-p^- +i\epsilon)(-p^- + k^- +i\epsilon)}
\bigg) 
\notag \\
- \frac{f^{b_3c_3e} f^{c_1ea}}{3! }
&\bigg(
      \frac{2}{(k^- +i\epsilon)(p^-  + i\epsilon)} 
      +
      \frac{2}{(-k^- +i\epsilon)(-p^-  + i\epsilon)} 
      \notag \\
      &
      -
      \frac{1}{(-k^- + i\epsilon)(p^- - k^- +i\epsilon)}
      -
      \frac{1}{(k^- + i\epsilon)(-p^- +k^-+i\epsilon)}
      \notag \\
      &
      -
      \frac{1}{(p^- +i\epsilon)(p^- - k^- +i\epsilon)}
      -
     \frac{1}{(-p^- +i\epsilon)(-p^- + k^- +i\epsilon)}
\bigg)
\end{align}
As far as the momentum structure is concerned, this can be compactified to
\begin{align}
  \label{eq:146}
  \frac{f^{b_3 c_1e} f^{c_3e a}}{k^- (p^- - k^-)} &+ \frac{f^{b_3c_3e} f^{c_1ea}}{k^- (-p^-) }  =
\notag \\
=\frac{f^{b_3 c_1e} f^{c_3e a}}{3!} 
&\bigg(
      \frac{4}{k^- (p^- - k^-)} 
      +
      \frac{2}{k^- p^- }
      +
      \frac{2}{p^- (p^- - k^- )}
\bigg) 
\notag \\
+ \frac{f^{b_3c_3e} f^{c_1ea}}{3! }
&\bigg(
      \frac{4}{(-k^- )p^-  } 
      +
      \frac{2}{(-k^- )(p^- - k^- )}
      +
      \frac{2}{p^- (p^- - k^- )}
\bigg)
\end{align}
while one has to keep in mind, that the pole structure is as given in eq. (\ref{eq:144}). Insert now this for a check into (\ref{eq:133}). We then find
\begin{align}
  \label{eq:147}
\tilde G_1 &= 
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2  ({\bm{k}}_1 + {\bm{k}}_2)^2}{p^2 (p-k_1 - k_2)^2}  
\bigg[
      \frac{1}{(p-k_1)^2}
      \notag \\
      &\frac{1}{6}\bigg(
                  \frac{4}{ (-k_1^- - k_2^-)} \frac{(p^-)^{\omega_2}}{p^-} 
                  +
                  \frac{2}{ (-k_1^- - k_2^-)} \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- -k_2^-} 
                  + 
                  2\frac{(p^-)^{\omega_2}}{p^-} \frac{(p^- - k_1^- - k_2^-)^{\tilde \omega_2}}{(p^- - k_1^- - k_2^-)}
                  \bigg)   
      \notag \\
      &+    
      \frac{1}{(p-k_2)^2} 
      \frac{1}{6}\bigg(
                 \frac{4}{k_1^- +k_2^-}\frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- - k_2^-}
                 +
                 \frac{2}{k_1^- +k_2^-} \frac{(p^-)^{\omega_2}}{p^-} 
                 +
                 2\frac{(p^-)^{\omega_2}}{p^-} \frac{(p^- - k_1^- - k_2^-)^{\tilde \omega_2}}{(p^- - k_1^- - k_2^-)}   \bigg)
\notag \\
&+
8g^4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\frac{{\bm{q}}^2 ({\bm{k}}_2 + {\bm{k}}_3)^2}{p^2 (p-q +k_1 )^2} 
\bigg[
     \frac{1}{(p-k_2)^2} 
     \notag \\ &
    \frac{1}{6} \bigg(
                      \frac{4}{  k_1^- }  \frac{(p^-)^{\omega_2}}{p^-}
                      +
                      \frac{2}{k_1^-} \frac{(p^- + k_1^- )^{\omega_2}}{p^- + k_1^-}
                      +
                      2\frac{(p^-)^{\omega_2}}{p^-}\frac{(p^- + k_1^-)^{\tilde \omega_2}}{p^- + k_1^-}
     \bigg)
     \notag \\
     &+ 
     \frac{1}{(p- q + k_1 +k_2)^2}
     \bigg(
          \frac{4}{  -k_1^- }      \frac{(p^- +k_1^-)^{\omega_2}}{p^- + k_1^- }
          +
          \frac{2}{-k_1^-} \frac{(p^-)^{\omega_2}}{p^-}
          +
          2\frac{(p^-)^{\omega_2}}{p^-}\frac{(p^- + k_1^-)^{\tilde \omega_2}}{p^- + k_1^-}
     \bigg)
\end{align}
Applying now shifts $p \to -p + k_1 + k_2$ and $p \to -p + q - k_1$ respectively one obtains
\begin{align}
  \label{eq:148}
\tilde G_1 &= 
8g^4  \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})   
\int \frac{d^4 p}{(2\pi)^4} (p^+)^{\omega_1}
\frac{{\bm{q}}^2  ({\bm{k}}_1 + {\bm{k}}_2)^2}{p^2 (p-k_1 - k_2)^2}  
\bigg[
      \frac{1}{(p-k_1)^2}
      \notag \\
      &\frac{1}{6}\bigg(
                  \frac{4}{ (-k_1^- - k_2^-)} \frac{(p^-)^{\omega_2}}{p^-} 
                  +
                  \frac{2}{ (-k_1^- - k_2^-)} \frac{(p^- - k_1^- - k_2^-)^{\omega_2}}{p^- - k_1^- -k_2^-} 
                  + 
                  2\frac{(p^-)^{\omega_2}}{p^-} \frac{(p^- - k_1^- - k_2^-)^{\tilde \omega_2}}{(p^- - k_1^- - k_2^-)}
                  \bigg)   
      \notag \\
      &+    
      \frac{1}{(p-k_1)^2} 
      \frac{1}{6}\bigg(
                 \frac{4}{k_1^- +k_2^-}\frac{(-p^- )^{\omega_2}}{-p^- }
                 +
                 \frac{2}{k_1^- +k_2^-} \frac{(-p^- + k_1^- + k_2^-)^{\omega_2}}{-p^- + k_1^- + k_2^-} 
                 +
                 2\frac{(-p^-)^{\tilde\omega_2}}{-p^-} \frac{(-p^- + k_1^- + k_2^-)^{ \omega_2}}{(-p^- + k_1^- + k_2^-)}   \bigg)
\notag \\
&+
8g^4 \tr(T^{a}T^{b_1}T^{b_2}T^{b_3})
\int \frac{d^4 p}{(2\pi)^4}  (p^+)^{\omega_1}
\frac{{\bm{q}}^2 ({\bm{k}}_2 + {\bm{k}}_3)^2}{p^2 (p-q +k_1 )^2} 
\bigg[
     \frac{1}{(p-k_2)^2} 
     \notag \\ &
    \frac{1}{6} \bigg(
                      \frac{4}{  k_1^- }  \frac{(p^-)^{\omega_2}}{p^-}
                      +
                      \frac{2}{k_1^-} \frac{(p^- + k_1^- )^{\omega_2}}{p^- + k_1^-}
                      +
                      2\frac{(p^-)^{\omega_2}}{p^-}\frac{(p^- + k_1^-)^{\tilde \omega_2}}{p^- + k_1^-}
     \bigg)
     \notag \\
     &+ 
     \frac{1}{(p- k_2)^2}
    \frac{1}{6} \bigg(
          \frac{4}{  -k_1^- }      \frac{(-p^- )^{\omega_2}}{-p^-  }
          +
          \frac{2}{-k_1^-} \frac{(-p^- - k_1^-)^{\omega_2}}{-p^- - k_1^-}
          +
          2\frac{(-p^- - k_1^-)^{\tilde \omega_2}}{- p^- - k_1^-}\frac{(-p^- )^{ \omega_2}}{-p^- }
     \bigg)
\end{align}
I am still not sure how the last term (the one with two omega-terms)
should be understood, as we are dealing in the present case only with
a single gluon loop integration. Apparently $p^-$ and $(p^- - k^-)$ are not independent. A possible solution would be to postulate that one has to re-write the denominators in a way that leaves only one 'loop'-denominator to be dealt with. In the present case this is easily possible. The crux is, wether this is possible in general and which price one pays for that. In the present case, we simply can use that
\begin{align}
  \label{eq:149}
& \frac{2}{(k^- +i\epsilon)(p^-  + i\epsilon)} 
      +
      \frac{2}{(-k^- +i\epsilon)(-p^-  + i\epsilon)} 
     % \notag \\
      %&
      -
      \frac{1}{(-k^- + i\epsilon)(p^- - k^- +i\epsilon)}
      -
      \frac{1}{(k^- + i\epsilon)(-p^- +k^-+i\epsilon)}
      \notag \\
      &
      -
      \frac{1}{(p^- +i\epsilon)(p^- - k^- +i\epsilon)}
      -
     \frac{1}{(-p^- +i\epsilon)(-p^- + k^- +i\epsilon)}
\notag \\
&=\frac{2}{(k^- +i\epsilon)(p^-  + i\epsilon)} 
      +
      \frac{2}{(-k^- +i\epsilon)(-p^-  + i\epsilon)} 
 -
      \frac{1}{(p^- +i\epsilon)( - k^- +i\epsilon)}
      -
     \frac{1}{(-p^- +i\epsilon)( k^- +i\epsilon)}
\notag \\
&=\bigg( \frac{2}{(k^- +i\epsilon)} - \frac{1}{-k^- + i\epsilon} \bigg) \frac{1}{(p^-  + i\epsilon)} 
      +
\bigg(      \frac{2}{(-k^- +i\epsilon)} - \frac{1}{k^- +i\epsilon} \bigg)\frac{1}{(-p^-  + i\epsilon)} 
\end{align}
Eq. (\ref{eq:148})  then turns into (\ref{eq:133}), but with the above convention for the $k^-$ integration.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% TeX-master: "thesis_notes"
%%% End: 


